Evaluation of Sampling Methods for Scatterplots

Given a scatterplot with tens of thousands of points or even more, a natural question is which sampling method should be used to create a small but "good" scatterplot for a better abstraction. We present the results of a user study that investigates the influence of different sampling strategies on multi-class scatterplots. The main goal of this study is to understand the capability of sampling methods in preserving the density, outliers, and overall shape of a scatterplot. To this end, we comprehensively review the literature and select seven typical sampling strategies as well as eight representative datasets. We then design four experiments to understand the performance of different strategies in maintaining: 1) region density; 2) class density; 3) outliers; and 4) overall shape in the sampling results. The results show that: 1) random sampling is preferred for preserving region density; 2) blue noise sampling and random sampling have comparable performance with the three multi-class sampling strategies in preserving class density; 3) outlier biased density based sampling, recursive subdivision based sampling, and blue noise sampling perform the best in keeping outliers; and 4) blue noise sampling outperforms the others in maintaining the overall shape of a scatterplot.

==> Evaluation of Sampling Methods archive/1-introduction.tex <==

\firstsection{Introduction}
\maketitle
% Scatterplots are one of the most \shixia{useful and powerful visual representations for analyzing multidimensional data~\cite{Sarikaya18}, which are widely used in multidimensional  data analysis.}
Scatterplots are one of the most widely used \shixia{visual representations in exploratory data analysis}~\cite{micallef2017towards,Sarikaya18}.
Their flexibility enables \doc{the discovery of} free-form patterns in \doc{two-dimensional} data, such as trends, clusters, and outliers~\cite{Kandogan12}.
% discovering
\doc{In conjunction with} dimensionality reduction approaches, scatterplots are also the dominant visualization tool \doc{for exploring} high-dimensional data~\cite{liu2019crowsourcing,Sacha17,sedlmair2013empirical}.
% With the companion of
% to explore
However, scatterplots become less effective when data grows in \lingyun{size}. %scale
First, the overdraw issue will \doc{adversely impact} the \doc{ability to comprehend} scatterplots~\cite{Mayorga13}.
% \lingyun{affect}
% understanding of
Second, the speed of \lingyun{producing visualization}, \ie, loading and rendering source data, will \doc{become} a considerable issue~\cite{Park2015}.
%be

\looseness=-1
\revision{
Many efforts have been devoted to addressing the overplotting issues in scatterplots, including sampling~\cite{Dix2002, Ellis2005}, abstraction~\cite{liu2017towards,Zhao2019phoenixmap}, modifying the size~\cite{Li2010size, Woodruff1998} and the opacity~\cite{Li2010lightness, Mayorga13} of the visual marks, and other hybrid methods~\cite{Matejka2015}.
However, many of them still suffer from the scalability problem~\cite{Ellis2007} since they still need to render a large number of data points or execute complex computations to produce the visualization, which restricts their practical use due to limited visualization capability of the display devices or computational resources.}
% Although the above methods can address the overplotting issue, many of them still suffer from the scalability problem~\cite{Ellis2007} since it still needs to render a large number of data points or execute complex computations to produce the visualization, which restricts their practical use by the visualization capability of the display devices or the limited computational resources.
To overcome the scalability issue in scatterplots, sampling has been well studied in data mining~\cite{Park2015} and visualization~\cite{Bertini2006, Chen14,yuan2021survey}.
Generally, sampling aims to select a statistically unbiased representation of the full dataset.
In different scenarios, many sampling strategies have been developed to enhance specific aspects of the full dataset, \eg, density~\cite{Bertini2006}, outlier~\cite{Xiang19}, \shixia{shape~\cite{Liu2017}}, and class ratio~\cite{Chen14, Chen20, Hu20}.
As shown in Fig.~\ref{fig:teaser}, the three sampling strategies preserve different features in their sampling results.
Rojas~\etal~\cite{Rojas17} interviewed 22 data scientists and concluded that random sampling, which is statistically unbiased, is the only \doc{appropriate} choice \doc{open to} these scientists for data exploration.
% of
Although other sampling strategies can provide different insights for data exploration, data scientists are not familiar with them, and \lingyun{they} do not know which strategy to use in a specific scenario.
For instance, \lingyun{although} \yuanjun{blue noise sampling} \lingyun{has been} widely used in computer graphics and visualization, we have not found \doc{examples of} its application in data mining in our literature review.
%Why scientists in data mining do not use blue-noise sampling?
%In which scenario it performs better than other sampling strategies?
%A study is required to evaluate these strategies and provide guidelines for choosing sampling strategies.

\looseness=-1
Nevertheless, the researches \doc{into} sampling strategy design have \doc{conducted} many quality comparisons.
% on
% performed
\doc{However,} performing a perception-based evaluation study is still essential \doc{for providing} guidelines \doc{for} choosing sampling strategies.
% to provide
% of
On the one hand, most of the existing comparisons are based on objective quality measures, \eg, density, class ratio, and \yuanjun{the} number of outliers.
Their conclusions may not be suitable for visualization tasks due to perceptual biases~\cite{Ma18, Wei20}.
On the other hand, these strategy-oriented evaluations are limited to a subset of tasks and approaches.
\shixia{Thus, a} comprehensive evaluation \shixia{of representative approaches} is missing.

In this paper, we conduct four experiments to study the effects of typical sampling strategies on 2D scatterplots.
%\doc{For}
% First, we \doc{selected} seven widely used or task-specific sampling strategies \doc{based on} a comprehensive literature review.
First, we select seven strategies based on a comprehensive literature review.
They are either widely used or task-specific sampling strategies that have specific goals.
% by
The strategies include random sampling~\cite{mukhopadhyay2008theory}, blue noise sampling~\cite{Cook1986}, density biased sampling~\cite{palmer2000density}, multi-class blue noise sampling~\cite{Chen14, wei2010multi}, outlier biased density based sampling~\cite{Xiang19}, multi-view Z-order sampling~\cite{Hu20}, and recursive subdivision based sampling~\cite{Chen20}.
Second, we identify four typical analytical tasks in multi-class \doc{scatterplot} analysis, including identifying relative \yuanjun{region} density, relative \yuanjun{class} density, outliers, and shapes.
% all-class, per-class
Third, we formulate \yuanjun{four} hypotheses based on our experience and literature review.
We hypothesize that
% (1) all other sampling strategies perform better than the baseline, i.e., random sampling, in relative density identification tasks;
(1) for a scatterplot without class information, all other sampling strategies perform better than \shixia{random sampling} in relative \yuanjun{region} density identification tasks in terms of accuracy and efficiency;
% (2) for a scatterplot with class information, all other sampling strategies perform better than \shixia{random sampling} in relative density identification tasks in terms of accuracy and efficiency;
\yuanjun{(2) for a scatterplot with class information, multi-class sampling strategies perform better than other sampling strategies in relative class density identification tasks in terms of accuracy and efficiency;}
(3) \shixia{outlier biased density based sampling is the best} in the outlier identification task;
% \doc{at}
(4) \shixia{blue noise sampling \yuanjun{and multi-class blue noise sampling} perform better than other strategies in preserving the overall shape.}

We select eight datasets that present different patterns and \lingyun{various degrees of visual clutter}.
%We conduct a series of experiments and recruited 100 participants
100 participants are recruited for the \lingyun{formal} experiments.
% We design objective questionnaires to present the tasks and record the accuracy and time to complete the tasks based on the results of different sampling strategies.
% We also design subjective questionnaires to observe subjective experience of the participants.
% Before the formal study, we perform preliminary studies to determine the sampling ratio and color stimuli.
% After that, we perform the formal study to collect experiments results.
Before the formal study, we perform a pre-study \lingyun{\doc{with} \yuanjun{160} participants} to determine the sampling ratio and color stimuli.
% on
% In the formal study, \lingyun{we \doc{conducted} a series of experiments on different sampling strategies and datasets and \doc{recorded} the \yuanjun{results} in completing these experiments.}
In the formal study, \lingyun{we conduct a series of experiments on different sampling strategies and datasets.}
% four
%we design objective questionnaires to present the tasks and record the accuracy and time to complete the tasks based on the results of different sampling strategies.
We also design subjective questionnaires to \lingyun{obtain} the subjective experience of the participants.
%\doc{better understand}
%observe
%Following the design, we perform the formal study to collect experiments results.

Based on the experiment results, we perform a comprehensive statistical analysis.
\yuanjun{The analysis results of the objective metrics} suggest that (1) \shixia{H1 is rejected;} with random sampling, participants use \doc{less} time to complete the \yuanjun{region} density identification tasks \jiazhi{with higher accuracy;}
%shorter
%two objective metrics
%more accurately; 
(2) H2 is partially confirmed; \jiazhi{multi-class sampling strategies \doc{achieved} higher accuracy than other strategies except for blue noise sampling; with random sampling, participants use \doc{less} time to complete the class density identification tasks.}
%shorter
%\yuanjun{with blue noise sampling, participants achieve comparable accuracy as with multi-class sampling strategies}, and with random sampling, participants use shorter time to complete the \yuanjun{class} density identification tasks; 
(3) H3 is \shixia{partially} confirmed; outlier biased density based sampling, recursive subdivision based sampling, and blue noise sampling \jiazhi{perform better than other strategies in identifying outliers.}
% \doc{at}
%are among the best to identify more outliers; 
(4) H4 is \yuanjun{partially} confirmed; \jiazhi{blue noise sampling performs the best in shape \doc{preservation} while multi-class blue noise sampling performs at a middle level.}
% preserving
%\yuanjun{multi-class blue noise sampling performs at an average level.}
The analysis results of the subjective questionnaires provide useful insights into the sampling strategies.
\lingyun{They disclose} subjective reasons for the objective metric results.
After the analysis, we summarize the ability of the seven sampling strategies to support our identified tasks.
% Finally, we discuss the limitations of this evaluation and future work.  By Shixia

In summary, we present a comprehensive perception-based evaluation of sampling strategies for scatterplots.
We contribute a carefully designed evaluation and a series of instructive findings, \doc{offering} guidelines for choosing sampling strategies in task-specific scenarios.
% \doc{have contributed}
% which provide 
\shixia{In addition, we also contribute a Python library for scatterplot sampling, which contains \yuanjun{14} commonly used sampling \lingyun{algorithms} and is available at} \url{https://github.com/libsampling/libsampling}.
% \url{http://bit.ly/2yWAzKI}.
% \url{http://shixialiu.com/libsampling/}
% \doc{have contributed}

==> Evaluation of Sampling Methods archive/2-related.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Related Work}
\label{sec:related-work}

\subsection{Sampling Strategies for Scatterplots}
\label{sec:categories}
% Scatterplots are the most common way to visualize high-dimensional data, but issues like visual clutters arise with the growing of volume of data.
% Sampling is an effective way to address the scalability problems of scatterplots, which reduce the amount of data.
% We mainly focus on the sampling techniques on two-dimensional multi-class scatterplots.
% The scatterplot sampling methods can be categorized based on two dimensions of sampling methods in data mining \cite{gu2000sampling}: (1) whether to consider class labels, and (2) whether the sampling probability of each point is equal.
\shixia{The scatterplot sampling methods can be categorized into two classes: single-class sampling and multi-class sampling.}

\vspace{1mm}
\noindent\textbf{Single-class sampling.}
% In real-world applications, class labels are common in data.
\shixia{This category of sampling strategies aims to preserve the properties of interest (\eg, density) of the original dataset without considering class information.}
Random sampling, the most widely used sampling method, is a classical single-class sampling method.
\shixia{It employs a \revision{\textbf{uniform sampling}} strategy that treats all samples equally and selects each sample with the same probability.}
% In this paper, \textbf{uniform sampling} refers to the sampling methods that assign equal probability to each point to be selected.

\looseness=-1
On the contrary, \revision{\textbf{non-uniform sampling}} strategies assign varying sampling probability to \lingyun{data} so that \lingyun{some specific properties of the original datasets can be better preserved.}
%they can better enhance some specific properties of the original dataset.
For example, in some cases, samples are required to be 
%\lingyun{more clearly} 
\jiazhi{better} spatially separated~\cite{Liu2017, zhang2014visual}.
Blue noise sampling~\cite{zhang2014visual, yan2015survey} achieves this by selecting samples with blue noise properties so that the selected samples will distribute 
%randomly and more 
evenly in the sample space.
%It \lingyun{rejects} samples that situate within a certain distance to the previously selected samples during the sampling process.
%so that the selected samples separate \lingyun{more clearly} in space.
Farthest point sampling~\cite{berger2016cite2vec} can also select samples with better \yuanjun{spatial} separation.
It randomly picks the first sample, and then \lingyun{iteratively} selects samples of maximal minimum distances to the previously selected ones.
Liu~\etal~\cite{Liu2017} developed a \jiazhi{dual space} sampling strategy. 
It computes a density field of the original sample space and maps the samples from the original density space to a uniform density space through a warping function.
Then it selects the samples via orthogonal least squares or weight sample elimination \jiazhi{in the mapped space} in order to maintain good spatial separation among the selected samples.
Lastly, the selected samples are mapped \jiazhi{back} into the original density space.

There are also sampling strategies \doc{that have been} developed to preserve density-related properties.
Density biased sampling~\cite{palmer2000density} tends to over-sample sparse regions and under-sample dense regions in the sample space.
It can counterbalance samples from both regions, thus preserving small clusters and more solitary samples.
% so that it can retain more points in the sparse regions.
Bertini~\etal~\cite{bertini2004chance, Bertini2006} proposed a non-uniform sampling strategy aiming at preserving the relative region density difference.
It divides the sample space into uniform grids, and then determines the represented density of each grid and finally selects samples from each grid according to \lingyun{the density}.
Joia~\etal~\cite{Joia2015} formulated the sampling problem as a matrix decomposition problem and solved it with singular value decomposition (SVD).
\lingyun{This method} performs SVD on the original dataset and selects the samples with the biggest correlation with top-$k$ basis vectors in the SVD result, where $k$ is a rank parameter indicating the number of principal components of interest.
The SVD based sampling strategy can counterbalance the number of points from regions with different densities.

% A number of outlier biased sampling strategies aim at preserving outliers in the original data, which are usually combined with other sampling strategies~\cite{liu2017visual, Xiang19}.
Outlier preservation is another common goal in sampling strategies.
A typical method \lingyun{for achieving this goal} is to alter \lingyun{existing} sampling strategies, making them probabilistically accept more outliers according to specified outlier scores~\cite{liu2017visual, Xiang19}.
For instance, Liu~\etal~\cite{liu2017visual} proposed outlier biased random sampling that assigns higher sampling probabilities to outliers in random sampling.
Xiang~\etal~\cite{Xiang19} increased the accepting probability of outliers in the sampling process of blue noise sampling and density biased sampling and developed outlier biased blue noise sampling and outlier biased density based sampling, respectively.
\lingyun{Moreover}, Cheng~\etal~\cite{Cheng2019} sampled the point clouds on their color mapping display using a hashmap based stratified sampling technique to preserve outliers while keeping the main distribution.
% \lingyun{This strategy} maintains a 2D hashmap during the sampling process to reduce the samples selected in dense regions and include more samples in sparse regions.

% In contrary, points have varying sampling probability in \textbf{non-uniform sampling}.
% For example, blue noise sampling~\cite{zhang2014visual, yan2015survey} will reject points that situate closer than a certain distance to the previously selected points during the sampling process, so that it will produce sampling results where sampled points are distributed more evenly.
% The overall sampling probability of each point is not equal, so it is a non-uniform sampling strategy.
% Farthest point sampling~\cite{berger2016cite2vec} is another strategy that makes the sampled points with blue noise properties.
% The biased sampling methods also fall into this category.
% Density-biased sampling~\cite{palmer2000density} tends to over-sample sparse regions and under-sample dense regions of the data so that it can retain more points in the sparse regions.
% An alternative non-uniform sampling method proposed by Bertini~\etal~\cite{bertini2004chance} bins regions with similar density and then samples points from each bin to achieve the similar goal.
% Joia~\etal~\cite{Joia2015} extracted representative instances from the original data, which was formulated it as a matrix decomposition problem and solved with singular value decomposition(SVD).
% Such SVD-based sampling method can also counterbalance the number of points from regions with different densities.
% Besides, outlier biased sampling strategies aim at preserving outliers in the original data, which are usually combined with other sampling strategies~\cite{liu2017visual, Xiang19}.
% By probabilistically accepting more outliers according to specified outlier scores, they can produce more outliers in their sampling results.
% Cheng~\etal~\cite{Cheng2019} sampled the point clouds on their color mapping display using a hashmap-based stratified sampling technique, which maintained most outliers while keeping the main distribution.


\begin{table}[t]
\vspace{1mm}
\caption{Characteristics of our collected sampling strategies. MC refers to multi-class sampling strategies; NU refers to non-uniform sampling strategies; S refers to considering spatial separation; D refers to considering density; O refers to considering outlier preservation. \revision{The selected sampling strategies are bold, and their acronyms are attached.}}
% The frequency of each strategy is in the brackets.
\vspace{-2mm}
\resizebox{0.49\textwidth}{!}{
\small
\renewcommand\arraystretch{1.2}
\centering
% \begin{minipage}{1\textwidth}
\revision{
% \begin{tabular}{|l|c|c|c|c|c|}
% \hline
% Sampling strategy & MC & NU & S & D & O \\
% \hline
% \textbf{Random sampling~(7)~\cite{dosSantosAmorim2012, Liu2016Grassmannian, Poco2011, Rieck2015, Tao2019, Xia2018, Zhao2020} (RS)} &  &  &  &  &  \\
% \hline
% \textbf{Blue noise sampling~(3)~\cite{Chen14, Xiang19, zhang2014visual} (BNS)} & & $\surd$ & $\surd$ & & \\
% \hline
% Farthest point sampling~(1)~\cite{berger2016cite2vec} & & $\surd$ & $\surd$ & & \\
% \hline
% Dual space sampling~(1)~\cite{Liu2017} & & $\surd$ & $\surd$ & & \\
% \hline
% \textbf{Density biased sampling (1)~\cite{palmer2000density, Xiang19} (DBS)} & & $\surd$ & & $\surd$ & \\
% \hline
% Non-uniform sampling~(2)~\cite{bertini2004chance, Bertini2006} & & $\surd$ & & $\surd$ & \\
% \hline
% SVD based sampling~(1)~\cite{Joia2015} & & $\surd$ & & $\surd$ & \\
% \hline
% Outlier biased random sampling~(2)~\cite{liu2017visual, Zhao2019} & & $\surd$ & & & $\surd$ \\
% \hline
% \textbf{Outlier biased density based sampling~(1)~\cite{Xiang19} (OBDBS)} & & $\surd$ & & $\surd$ & $\surd$ \\
% \hline
% Outlier biased blue noise sampling~(1)~\cite{Xiang19} & & $\surd$ & $\surd$ & & $\surd$ \\
% \hline
% Hashmap based sampling~(1)~\cite{Cheng2019} & & $\surd$ & & & $\surd$ \\
% \hline
% \textbf{Multi-class blue noise sampling~(1)~\cite{Chen14, wei2010multi} (MCBNS)} & $\surd$ & $\surd$ & $\surd$ & & \\
% \hline
% \textbf{Multi-view Z-order sampling~(1)~\cite{Hu20} (MVZS)} & $\surd$ & $\surd$ & & $\surd$ & \\
% \hline
% \textbf{Recursive subdivision based sampling~(1)~\cite{Chen20} (RSBS)} & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ \\
% \hline
% \end{tabular}
% \begin{tabular}{|l|l|c|c|c|c|c|c|}
% \hline
% Sampling strategy & Ref. & Fre. & MC & NU & S & D & O \\
% \hline
% \textbf{Random sampling (RS)} & \makecell[l]{\cite{dosSantosAmorim2012},\cite{Liu2016Grassmannian}, \cite{Poco2011}, \cite{Rieck2015}, \\ \cite{Tao2019}, \cite{Xia2018}, \cite{Zhao2020}} & 7 &  &  &  &  &  \\
% \hline
% \textbf{Blue noise sampling (BNS)} & \cite{Chen14}, \cite{Xiang19}, \cite{zhang2014visual} & 3 & & $\surd$ & $\surd$ & & \\
% \hline
% Farthest point sampling & \cite{berger2016cite2vec} & 1 & & $\surd$ & $\surd$ & & \\
% \hline
% Dual space sampling & \cite{Liu2017} & 1 & & $\surd$ & $\surd$ & & \\
% \hline
% \textbf{Density biased sampling (DBS)} & \cite{Xiang19} & 1 & & $\surd$ & & $\surd$ & \\
% \hline
% Non-uniform sampling & \cite{bertini2004chance}, \cite{Bertini2006} & 2 & & $\surd$ & & $\surd$ & \\
% \hline
% SVD based sampling & \cite{Joia2015} & 1 & & $\surd$ & & $\surd$ & \\
% \hline
% Outlier biased random sampling & \cite{liu2017visual}, \cite{Zhao2019} & 2 & & $\surd$ & & & $\surd$ \\
% \hline
% \textbf{Outlier biased density based sampling (OBDBS)} & \cite{Xiang19} & 1 & & $\surd$ & & $\surd$ & $\surd$ \\
% \hline
% Outlier biased blue noise sampling & \cite{Xiang19} & 1 & & $\surd$ & $\surd$ & & $\surd$ \\
% \hline
% Hashmap based sampling & \cite{Cheng2019} & 1 & & $\surd$ & & & $\surd$ \\
% \hline
% \textbf{Multi-class blue noise sampling (MCBNS)} & \cite{Chen14} & 1 & $\surd$ & $\surd$ & $\surd$ & & \\
% \hline
% \textbf{Multi-view Z-order sampling (MVZS)} & \cite{Hu20} & 1 & $\surd$ & $\surd$ & & $\surd$ & \\
% \hline
% \textbf{Recursive subdivision based sampling (RSBS)} & \cite{Chen20} & 1 & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ \\
% \hline
% \end{tabular}
\begin{tabular}{|l|l|c|c|c|c|c|}
\hline
Sampling strategy & Works & MC & NU & S & D & O \\
\hline
\textbf{Random sampling (RS)} & \makecell[l]{\cite{dosSantosAmorim2012}, \cite{Liu2016Grassmannian}, \cite{Poco2011}, \cite{Rieck2015}, \\ \cite{Tao2019}, \cite{Xia2018}, \cite{Zhao2020}}  &  &  &  &  &  \\
\hline
\textbf{Blue noise sampling (BNS)} & \cite{Chen14}, \cite{Xiang19}, \cite{zhang2014visual}  & & $\surd$ & $\surd$ & & \\
\hline
Farthest point sampling & \cite{berger2016cite2vec}  & & $\surd$ & $\surd$ & & \\
\hline
Dual space sampling & \cite{Liu2017}  & & $\surd$ & $\surd$ & & \\
\hline
\textbf{Density biased sampling (DBS)} & \cite{Xiang19}  & & $\surd$ & & $\surd$ & \\
\hline
Non-uniform sampling & \cite{bertini2004chance}, \cite{Bertini2006}  & & $\surd$ & & $\surd$ & \\
\hline
SVD based sampling & \cite{Joia2015}  & & $\surd$ & & $\surd$ & \\
\hline
Outlier biased random sampling & \cite{liu2017visual}, \cite{Zhao2019}  & & $\surd$ & & & $\surd$ \\
\hline
\textbf{Outlier biased density based sampling (OBDBS)} & \cite{Xiang19}  & & $\surd$ & & $\surd$ & $\surd$ \\
\hline
Outlier biased blue noise sampling & \cite{Xiang19}  & & $\surd$ & $\surd$ & & $\surd$ \\
\hline
Hashmap based sampling & \cite{Cheng2019}  & & $\surd$ & & & $\surd$ \\
\hline
\textbf{Multi-class blue noise sampling (MCBNS)} & \cite{Chen14}  & $\surd$ & $\surd$ & $\surd$ & & \\
\hline
\textbf{Multi-view Z-order sampling (MVZS)} & \cite{Hu20}  & $\surd$ & $\surd$ & & $\surd$ & \\
\hline
\textbf{Recursive subdivision based sampling (RSBS)} & \cite{Chen20}  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ \\
\hline
\end{tabular}
}
}
% \end{minipage}
\label{tab:category}
\vspace{-7mm}
\end{table}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fig/datasets_rev.pdf}
\vspace{-5mm}
\caption{Datasets selected for our evaluation. \revision{All datasets are multi-class data. The color encodes the labels.} The numbers in the brackets indicate the sizes of the datasets.}
\vspace{-5mm}
\label{fig:datasets}
\end{figure*}

\vspace{1mm}
\noindent\textbf{Multi-class sampling.}
% Unlike single-class sampling strategies, multi-class sampling strategies need to take the class labels of the data as input, and they are mostly non-uniform sampling strategies.
% Unlike single-class sampling strategies, multi-class sampling strategies need to take the class labels of a dataset as input.
% \shixia{They aim to preserve the properties of interest (\eg, density) of each individual class as well as their union.}
Unlike single-class sampling strategies, multi-class sampling strategies aim to preserve the properties of interest (\eg, density) of each individual class as well as their union.
\revision{Thus, all the multi-class sampling methods are \textbf{non-uniform}.}
Wei~\cite{wei2010multi} extended blue noise sampling to multi-class scenarios to maintain the blue noise properties of \lingyun{each class of samples and of the whole dataset}.
Based on the multi-class blue noise sampling, Chen~\etal~\cite{Chen14} employed a hierarchical sampling strategy that selects samples round by round.
It first selects samples from the coarsest level using multi-class blue noise sampling, and when the selected samples are not enough, it reduces the restricted distance of the selected samples by half and adds more samples in the final result.
Recently, a recursive subdivision based sampling strategy proposed by Chen~\etal~\cite{Chen20} \doc{met} several requirements \doc{for} multi-class scatterplot exploration, including preserving relative densities, maintaining outliers, and minimizing visual artifacts.
% in
It splits the visual space into a binary KD-tree and determines which class of instances should be selected at each leaf node based on relative class density by a backtracking procedure.
Additionally, Hu~\etal~\cite{Hu20} developed multi-view Z-order sampling based on Z-order curve methods~\cite{Zheng2013} and formulated it as a set cover problem.
The sets were constructed by segmenting the Z-order curves of the samples in each class and the whole dataset, respectively.
\lingyun{This strategy} selects samples by greedily solving such set cover problems and gets satisfying results in terms of minimizing kernel density estimation error.


% Wei~\cite{wei2010multi} proposed multi-class blue noise sampling, based on which Chen~\etal~\cite{Chen14} developed a hierarchical sampling technique to visualize multi-class scatterplots.
% Some recent works focused on developing multi-class sampling methods and achieved satisfying results on a variety of datasets.
% For example, Chen~\etal~\cite{Chen20} proposed a recursive sampling technique based on KD-tree.
% They first split the visual space into a binary KD-tree and then determined which class of instances should be selected at each leaf node by a backtracking process.
% Hu~\etal~\cite{Hu20} formulated the sampling problem in multi-class scatterplots as a set cover problem, where such sets were constructed by segmenting the Z-orders for the instances of each class and all instances, respectively.
% A sampling result can be obtained by greedily solving this problem.
% Some recent works developed multi-class sampling methods, such as multi-view Z-order sampling and recursive subdivision based sampling, achieved satisfying results on a variety of datasets.

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{fig/category.png}
% \caption{Categories of our collected sampling methods.}
% \label{fig:category}
% \end{figure}
% \begin{table*}[htb]
% \renewcommand\arraystretch{1.2}
% \centering
% \caption{Categories of our collected sampling methods.}
% \begin{tabular}{|l|l|l|}
% \hline
% Type & Single-class sampling & Multi-class sampling \\
% \hline
% Uniform sampling & Random sampling~\cite{Zhao2020, dosSantosAmorim2012, Poco2011, Xia2018} &  \\
% \hline
% \multirow{9}{*}{Non-uniform sampling} & Blue noise sampling~\cite{zhang2014visual, Xiang19} & \\
% &  Farthest point sampling~\cite{berger2016cite2vec} & \\
% &  OD-UD sampling~\cite{Liu2017} & \\
% \cline{2-2}
% &  Density biased sampling~\cite{Xiang19, palmer2000density} & Multi-class blue noise sampling~\cite{wei2010multi, Chen14} \\
% &  SVD based sampling~\cite{Joia2015} & Multi-view Z order sampling~\cite{Hu20} \\
% \cline{2-2}
% & Outlier biased random sampling~\cite{liu2017visual, Zhao2019} & Recursive subdivision based sampling~\cite{Chen20} \\
% & Outlier biased blue noise sampling~\cite{Xiang19} & \\
% & Outlier biased density based sampling~\cite{Xiang19} & \\
% & Hashmap-based stratified sampling~\cite{Cheng2019} & \\
% \hline
% \end{tabular}
% \label{tab:category}
% \vspace{-3mm}
% \end{table*}

% The simplest way to sample a subset from data is random sampling, which selects each instance with equal probability.
% However, the result of random sampling can be annoyed with irregularly overlapping samples and space-wasting.
% Blue noise sampling is a solution to this phenomenon that it constrains the minimal distance among the selected instances to produce samples distributed more uniformly.
% Farthest point sampling used in~\cite{} can also generate samples with blue noise properties.
% More sampling strategies that sample different instances with different probabilities are developed in order to achieve some individual goals.
% Density-biased sampling selects instances in sparse regions with higher probability, and vice versa, in order to balance the instances sampled from dense and sparse regions.
% SVD-based sampling and non-uniform sampling can also preserve samples from the sparse regions.
% Some other sampling strategies aim at preserving more outliers in the sampling process.
% Liu~\etal and Xiang~\etal achieved this by simply assigning higher sampling probability to the instances with higher outlier scores.
% They enhanced common sampling strategies (e.g., random sampling) in such an outlier-biased way, and developed outlier-biased random sampling, outlier-biased blue noise sampling and, outlier-biased density-based sampling.
% Besides, Cheng~\etal sampled the point clouds on their color mapping display using a hashmap-based stratified sampling technique, which maintained most outliers while keeping the main distribution.

% The aforementioned sampling strategies do not consider the class labels of the data instances, but the latest works leverage them for better sampling results.
% Wei proposed multi-class blue noise sampling, based on which Chen~\etal developed a hierarchical sampling technique to visualize multi-class scatterplots.
% Recently, some specific data structures are introduced to develop new sampling techniques.
% Chen~\etal proposed a recursive sampling technique based on KD-tree.
% They first split the visual space into a binary KD-tree and then determined which class of instances should be selected at each leaf node by a backtracking process.
% Hu~\etal formulated the sampling problem in multi-class scatterplots as a set cover problem, where such sets were constructed by segmenting the Z-orders for the instances of each class and all instances, respectively.
% A sampling result can be obtained by greedily solving the set cover problem.

% \subsection{Evaluations of Sampling and Scatterplots}
\subsection{Evaluation Studies of Sampling Methods}
% Given the widely used nature of scatterplots in visualization, some measures have been proposed to describe the features of scatterplots~\yuanjun{[cite]},
% However, these measures cannot always fit in with the human perception~\yuanjun{[cite]}, and many efforts have explored the design of scatterplots in terms of perception by empirical evaluation.
% For example, Wei~\etal evaluated the perceptual bias of numerosity, correlation, and cluster separation with scaling scatterplots.
% Lu~\etal assigned winglets to the points on the multi-class scatterplots to visualize their uncertainty and evaluated the enhancement brought by their design using scatterplots with different numbers of clusters and cluster overlaps.

% There are also user studies conducted to demonstrate the effectiveness of the proposed sampling methods~\yuanjun{[cite]}.
% Both hierarchical multi-class blue noise sampling~\yuanjun{[cite]} and multi-view Z-order sampling~\yuanjun{[cite]} were compared with the previous forms of visualization to show their performances on recognition of data classes and densities.

% Existing evaluation works considering a specific setting (e.g., graph sampling, a type of sampling methods)

A few \doc{previous} studies paid attention to the evaluation of sampling methods.
\lingyun{However, they} either \doc{evaluated} the sampling methods in certain situations (\eg, graph sampling) or \doc{evaluated} a specific sampling method to show its capability.
% have, before

\vspace{1mm}
\looseness=-1
\noindent\textbf{Generic Evaluation}.
Previous studies concentrated on evaluating sampling methods for graph data~\cite{wu2016evaluation, nguyen2017proxy}.
Wu~\etal~\cite{wu2016evaluation} conducted a survey on graph sampling methods and performed an empirical evaluation \doc{of} the preservation of the three most important visual factors on five selected methods.
% about
Later, Nguyen~\etal~\cite{nguyen2017proxy} proposed a family of quality metrics to evaluate the stochastic graph sampling methods in an objective manner.

\vspace{1mm}
\noindent\textbf{Instance-oriented Evaluation}.
% Specific Evaluation
When proposing new sampling methods, researchers \doc{also conduct} evaluations to demonstrate their effectiveness.
% would
Some of them used quality measures to make a quantitative evaluation in terms of data features.
Chen~\etal~\cite{Chen20} adopted four measures based on their design requirements and compared their results with three baseline methods.
They also presented three case studies to show the usefulness of their method in multi-dimension data analysis.
However, as numerical measures \lingyun{do not always agree with} human perception~\cite{wang2019improving}, other efforts focused on empirically evaluating perceptual subjects through user studies.
For example, both hierarchical multi-class blue noise sampling~\cite{Chen14} and multi-view Z-order sampling~\cite{Hu20} employed user studies  to confirm their superiority \doc{in} the recognition of data classes and densities.
% on

\looseness=-1
To the best of our knowledge, there has never been a systematic evaluation of sampling on scatterplots from the perspective of visualization.
% Inspired by~\cite{wu2016evaluation}, 
In this paper, we collect the representative sampling strategies on scatterplots from the visualization community and then conduct four experiments to evaluate their ability to retain data features on perception.



==> Evaluation of Sampling Methods archive/3-hypotheses.tex <==
\section{Evaluation Landscape}
\label{sec:Hypothesis}
% Sampling is described in the literature as being useful and effective for addressing scalability issues in scatterplot-based data exploration and analysis.
% As many sampling strategies have been developed for different types of applications, users face the challenge of selecting the right strategy in a specific scenario.
% To address this challenge, we aim to evaluate the performance and capability of commonly used sampling strategies.


\looseness=-1
% Based on a comprehensive literature review, we \doc{selected} a set of representative sampling strategies, datasets, and visual factors to be included in our evaluation.
% evaluated.

\subsection{Selection of Sampling Strategies}
\label{sec:SelectionOfSamplingMethods}

% \subsubsection{Paper Collection}
% \noindent\textbf{Paper collection}.
To comprehensively summarize the sampling strategies used in the visualization community, we first surveyed papers from 
\jiazhi{the journal of IEEE TVCG and three mainstream visualization conferences (IEEE VIS, PacificVis, and EuroVis)}
%top journal(IEEE TVCG) and three top conferences (IEEE VIS, PacificVis, and EuroVis) 
published from 2010 to 2019.
% \doc{from}
We used Google Scholar to search for the papers with the keyword "sampling" from the \doc{above sources}.
There are 1,562 papers in the initial result.
%\jiazhi{were} 
\lingyun{Next, we filtered out papers \doc{that} are not relevant to sampling in visualization.}
% which are
\lingyun{We kept papers that either applied sampling for visualization purposes or proposed new sampling strategies in visual analytics or information visualization.}
Finally, \lingyun{\yuanjun{25} papers remained in our survey. We further summarized the sampling strategies discussed in these papers}.

% \subsubsection{Category of Sampling Methods}

% The sampling methods used in visualization can be categorized based on two dimensions of sampling methods in data mining~\yuanjun{[cite]}: (1) whether the sampling probability of each point is equal, and (2) whether to consider class labels.

% \textbf{Uniform sampling.}
% In our paper, uniform sampling refers to the sampling methods that assign equal probability to each point to be selected.
% Such sampling strategies preserve relative densities of the original data to some extent, but they can cause visual clutters.
% Random sampling, the most widely used sampling method, is just a kind of uniform sampling.
% Another sampling methods lie in this category is systematic sampling, which selecting points at regular intervals through an ordered list.

% \textbf{Non-uniform sampling.}
% Contrary to uniform sampling, points have varying sampling probability in non-uniform sampling.
% Blue noise sampling and farthest point sampling can produce sampling results where sampled points are distributed more evenly.
% Many biased sampling methods also fall into this category.
% Density-biased sampling~\yuanjun{[cite]} tends to over-sample sparse regions and under-sample dense regions so that it can retain more points in the sparse regions.
% An alternative non-uniform sampling method proposed by Bertini~\etal~cite{xxx} bins regions with similar density and then samples points from each bin to achieve the same goal.
% Besides, outlier biased sampling strategies aim at preserving outliers in the original data, which are usually combined with other sampling strategies.
% By probabilistically accepting more outliers according to specified outlier scores, they can produce more outliers in their sampling results.

% \textbf{Single-class sampling.}
% % In real-world applications, class labels are common in data.
% Obviously, the sampling methods mentioned above do not consider the class labels of the points during the sampling process, so they are regarded as single-class sampling methods.
% However, they can also perform sampling on multi-class data, which is common in real-world applications, by treating all the points as the same class.

% \textbf{Multi-class sampling.}
% Multi-class sampling methods need to take class labels as input.
% Multi-class blue noise sampling proposed by Wei~\yuanjun{[cite]} preserved the blue noise properties of points of each class separately.
% Some recent works developed multi-class sampling methods, such as multi-view Z-order sampling~\yuanjun{[cite]} and recursive subdivision based sampling~\yuanjun{[cite]}, achieved satisfying results on a variety of datasets.
% \vspace{1mm}
% \subsubsection{Methods Selection}
% \noindent\textbf{Methods Selection}
The collection of the sampling strategies are \yuanjun{listed} in Table~\ref{tab:category}.
%, where the categories of them are the same as in Section~\ref{sec:categories}.
%\lingyun{Since there are diverse sampling methods used for visualization purposes and obviously it is \yuanjun{impractical} to evaluate all of them.}
% not realistic
\lingyun{We decided to focus on the widely used or} %state-of-the-art 
\jiazhi{recently advanced} \yuanjun{task-specific}
\lingyun{sampling strategies since there are diverse sampling strategies used for different visualization purposes, and it is obviously \yuanjun{impractical} to evaluate all \doc{of them} in our work.}
% \jiazhi{As a result,} \yuanjun{we selected} sampling strategies \yuanjun{that} have covered all the categories \revision{(\ie, single-class/multi-class sampling dimension and uniform/non-uniform sampling dimension)} for our evaluation.
\revision{As a result, we selected sampling strategies that cover all four categories in two dimensions, single-class/multi-class sampling and uniform/non-uniform sampling.}
% \revision{These sampling strategies have also covered all factors listed in Table~\ref{tab:category}.}
% \jiazhi{listed in Table~\ref{tab:category}}
We first selected random sampling (RS)~\cite{mukhopadhyay2008theory}, because it is the most widely used sampling strategy.
%, is selected as our baseline method.
We also selected other representative strategies, including blue noise sampling (BNS)~\cite{Cook1986}, density biased sampling (DBS)~\cite{palmer2000density}, and multi-class blue noise sampling (MCBNS)~\cite{Chen14, wei2010multi}.
In addition, outlier biased density based sampling (OBDBS)~\cite{Xiang19}, multi-view Z-order sampling (MVZS)~\cite{Hu20}, and recursive subdivision based sampling (RSBS)~\cite{Chen20} are selected, \revision{since they are reported to} perform the best in terms of their design requirements \revision{based on the experiment results from the previous studies}, respectively.
% those \lingyun{strategies} that
\revision{
% For instance, recursive subdivision based sampling~\cite{Chen20} outperforms the baseline sampling strategies in preserving relative class density and outliers, and is comparable with the best strategy in preserving relative region density with some numerical measures.
For instance, outlier biased blue noise sampling outperforms four other sampling methods in terms of preserving outliers and class consistency in the experiment~\cite{Xiang19}.}
These seven strategies \doc{have} all \doc{been} \yuanjun{included} in our study.
%They are also selected in our study.

\subsection{Selection of Datasets}
\looseness=-1
%To improve the trustworthiness of our evaluation results,
\lingyun{To ensure the reliability of the evaluation results,}
we selected datasets from the previous studies in visualization as our experiment data.
\lingyun{More specifically, we collected datasets that were used in the works in our survey.}
\lingyun{Since} most of them are high-dimensional data,
\lingyun{we first transformed them into 2D \yuanjun{data} using t-SNE and normalized \yuanjun{them} to $[0, 1] \times [0, 1]$.}
%they are transformed into 2D space using t-SNE and normalized to $[0, 1] \times [0, 1]$.
\lingyun{In the results, points} are located 
\jiazhi{as clusters in different shapes}
%\yuanjun{as clusters or as manifolds} 
in the obtained multi-class scatterplots.
%occur
In addition, the number of points and the clutter degrees of these scatterplots vary within a wide range.
According to the observations above, we selected eight representative datasets \yuanjun{shown in Fig.~\ref{fig:datasets}} with different characteristics: \lingyun{six datasets} where points are located as clusters (\emph{Swiss Roll 2D}~\cite{SwissRoll04}, \emph{Condition Based Maintenance}~\cite{Coraddu2014}, \emph{Crowdsourced Mapping}~\cite{Johnson2016}, \emph{MNIST}~\cite{Lecun1998}, \emph{Clothes}~\cite{Xiang19}, and \emph{Epileptic Seizure}~\cite{Andrzejak2001}); and two where points are located as 
%manifolds 
\jiazhi{curved stripes}
(\emph{Swiss Roll 3D}~\cite{SwissRoll04} and \emph{Abalone}~\cite{Dua2019}).
% \lingyun{finally}
% TODO citation
The clutter degrees of them vary from slight to severe as the order listed in each bracket.
\lingyun{The number of points in the selected datasets} ranges from thousands to tens of thousands, \yuanjun{as listed in Fig.~\ref{fig:datasets}}.

% 1) The process of our survey

% 2) The categorization of our sampling methods (orthogonal categories, jiazhi)
%     2.1)single class / multi class
%     2.2)uniform probability / non-uniform probability
\subsection{Selection of Visual Factors}
\label{sec:factor}
\looseness=-1
We identified the most critical visual factors for the sampling strategies by comprehensively reviewing existing works on sampling and scatterplots.
% \yuanjun{An earlier work propose several measures to assess scatterplots in five aspects, including outliers, shape, trend, density and coherence~\cite{Wilkinson2005}.}
% graph-theoretic measures
% we extracted the \emph{design requirements} and the \emph{application goals} of the sampling methods from our survey.
% \lingyun{make sure these two phrases}
% As visual clutter reduction is common in sampling, we did not take it into consideration. \lingyun{not very convincing, because it is common, so we did not take into consideration?}
\shixia{Previous studies have shown \lingyun{that} there are basically five goals related to scatterplot exploration, \yuanjun{including} outlier identification, shape examination, trend analysis, density detection, and coherence analysis~\cite{micallef2017towards,Wilkinson2005}.}
\yuanjun{In order to determine which of these factors mentioned in the aforementioned goals are \shixia{concerned in the existing sampling strategies},}
\shixia{we carefully \doc{examined} the \yuanjun{25} selected papers and extracted the visual factors that are considered in these works.}
% In the selected papers,
\shixia{Specifically,}
outlier maintenance is mentioned \doc{most often}, \doc{as it} appears in seven \yuanjun{out of the 25 papers}.
% the most
% which
\lingyun{Three papers concern preserving} the relative density and \lingyun{two concern} the overall shape of a scatterplot, respectively.
\revision{Here, \emph{the overall shape} refers to the geometric properties of the distribution of samples on a scatterplot, \eg, whether a set of scatter points are convex or not.}
% about
As a result, in the study, we decided to investigate the capabilities of different sampling strategies in preserving \textbf{outliers}, \textbf{density}, and the \textbf{overall shape} of a scatterplot.
% \lingyun{did you mention how many papers in total?} \yuanjun{Yes, in section 3.1.1, now also mentioned above}
% These three visual factors are of interest to visualization researchers in the sampling for scatterplots.
% Since numerical measurements are not always consistent with human perception~\cite{wang2019improving}, we intend to design experiments to evaluate the preservation of them from the perspective of perception.


==> Evaluation of Sampling Methods archive/4-pre-study.tex <==
\section{Pre-Study}
\looseness=-1
The purpose of the pre-study is to specify two experiment choices for the formal study: (1) how many points should be sampled from each dataset, and (2) 
\jiazhi{whether color encoding should be used in the experiment \doc{for} comparing region densities of multi-class scatterplots in the formal study.}
\jiazhi{\emph{Region density} refers to the density of data points regardless of class information.}
% \lingyun{We conducted two experiments to answer the \doc{respective questions}}.

%of
%whether color should be preserved in the \lingyun{experiment} of comparing \yuanjun{all-class} density \lingyun{of the sampling methods in the formal study}. %task
% above, respectively
% First of all, since the characteristics and the clutter degrees differ from dataset to dataset, it is necessary to recognize the number of points to be sampled from each dataset.
% As an irrelevant factor in the comparison of global density, color can interfere the human perception.
% To figure out the perceptual effect of color will help to determine whether it should be preserved in this task.

% \subsection{Design and Procedure}

% Two tasks were designed to answer the questions above, respectively. Participants were required to complete the tasks on our implemented web prototype. A questionnaire about the participants' background and their feedback on the tasks was attached to the end of the prototype.

% \textbf{T1: Sampling number identification.}
% This task aims at determining the proper sampling number of each dataset. Participants are asked to select a sampled scatterplot that still looked like the original one with the minimal number of points for each dataset.
% As Weber-Fechner Law states that the perceived intensity is proportional to the logarithm of the stimulus~\cite{portugal2011weber}, we then adopt a seven-level sampling results with $500$, $500*1.5$, $500*1.5^2$,..., $500*1.5^6$ points (a geometric sequence) by random sampling.
% %sample size
% Besides, a previous work ~\cite{} showed that different sampling techniques will produce very similar results with a sampling rate greater than 50\%, so we also limit the number of sample points to no more than half of the original data.

% \textbf{T2: Global density comparison.}
% We want to understand the effect of color when comparing global density.
% This task adopted a within-subject design, and the only variable here was whether the scatterplot was colored or not.
% Participants were asked to compare the average point density of two given regions in the same scatterplot and select the region with larger density quickly and accurately.
% We generated ten synthetic datasets using mixed Gaussian distributions with 3 to 10 classes, of which each had two different questions.
% Thus, 20 different questions were tested in total, and each question would be asked twice, once with a colored scatterplot and the other with an uncolored one.
% Average completion time and accuracy will be calculated in this task.

% \subsection{Results}

% We recruited 165 participants (134 males, 31 females, aged 18 - 60 years) for the preliminary study.
% All of them are either students with computer science backgrounds or researchers, and 65 out of them reported experience with sampling.
% It took about 10 minutes for each participant to finish the preliminary study.

% Given the fact that when there are more points in the sampled scatterplot, it will look more like the original scatterplot, We consider the proper number of points to sample from the original dataset should satisfy at least 80\% participants.
% In other words, more than 80\% of the participants select a number no more than it.
% Fig.~\fig{xxx} presents the results of T1, where the proper sampling number for most datasets is 2531.
% Exceptions exist in the dataset \emph{Clothes} and \emph{Epileptic Seizure}, both of which are required to sample 3796 points.
% This implies that more points are needed to be sampled in a scatterplot of a higher clutter degree in order to keep the sampling result close to it perceptually.
% Another exception arises in the dataset \emph{Abalone} containing only about 5000 points, while other datasets all contain more than 10000 points.
% Therefore, its proper sampling number is less correspondingly.
% As for the factor for similarity, over 75\% of them took the overall shape of each class of points into consideration, followed by density and outliers.

% The results of T2 is shown in Table~\tab{xxx}.
% The average accuracy of the colored and uncolored questions are 92.9\% and 93.3\%, respectively.
% No statistical significance in the difference of their accuracy is reported through hypothetical tests.
% However, the completion time of the uncolored questions is 235ms fewer than that of the colored ones on average.
% Since the completion time data are not subject to the normal distribution by the Shapiro-Wilk test, we conduct a Wilcoxon test to check for the significance of the time difference with the significance level $\alpha = 0.05$.
% The p-value of this test is less than 0.001, which means that such difference is statistically highly significant.
% In the questionnaire, participants were also asked to rate the color deficiency in T2 by a five-point Likert scale.
% The average score is 2.03, indicating that color affects the global density comparison slightly, which is coherent with our numerical result.
% A participant also commented that \emph{"the salient color may have an influence on my judgment of density"}.
% Consequently, in the formal study, we remove color in this task to eliminate the deficiency caused by color.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/interface1_new.pdf}
\vspace{-5mm}
\caption{Interface of Experiment 1 in the pre-study: the original scatterplot is located at the top-left, with the sampling results of increasing sampling number at the following positions.}
\vspace{-5mm}
\label{fig:interface_1}
\end{figure}

\subsection{Experiment 1: Sampling Number Identification}
\looseness=-1
We conducted a subjective experiment to specify the proper number of sampling points for each dataset.
On the one hand, we want set a small sampling number to clearly show the motivation of sampling, \yuanjun{\ie}, addressing the issue of visual clutter.
%\doc{the sampling}
On the other hand, the patterns of the original scatterplots will not be preserved if the sampling number is too small.
Because the patterns are different in different datasets, it is essential to choose a proper sampling number for each dataset.

%This experiment aims at selecting the proper sampling number for each dataset.
%Since the characteristics and the \lingyun{clutter degrees change} differ from dataset to dataset, it is necessary to recognize the number of points to be sampled from each dataset.
%\lingyun{Due to the different patterns and degrees of visual clutter, it is essential to choose a proper sampling number for each dataset.}

% \subsubsection{Task and Procedure}

\vspace{1mm}
\noindent\textbf{Task and Procedure}.
%The datasets we used were the same as those in the formal study.
We used the same \jiazhi{eight} datasets as those in the formal study.
%In the study, 
For each dataset, we showed the participants the original scatterplot as well as a series of sampled scatterplots with different sampling numbers.
Participants were asked to select \lingyun{the sampled scatterplot that has the smallest number of points while being perceptually similar to the original} \jiazhi{scatterplot.} %dataset}.
%\lingyun{Given the fact that the more points kept in the sampled scatterplot, the more similar it looks to the original scatterplot, we tried to find out the one that has the smallest number of points while being perceptually similar to the original dataset. Thus, participants were asked to select such a sampled scatterplot which contains the minimal number of points but still looks similar as the original scatterplot.}
Weber-Fechner Law states that the perceived intensity is proportional to the logarithm of the stimulus~\cite{portugal2011weber}. 
Therefore, we adopted a seven-level sampling with $500$, $500 \times 1.5$, $500 \times 1.5^2$, ..., $500 \times 1.5^6$ points (a geometric sequence) by \lingyun{random sampling}.%, the baseline sampling method}.
\jiazhi{We \doc{chose} random sampling because it has no preference for \revision {preserving} certain \doc{properties} of \doc{the} datasets.}
\revision{In addition, random sampling will not introduce bias to the sampled data statistically and guarantee the representativeness of the sampled data~\cite{verma2019statistics}.}
% \lingyun{why by random sampling}
%sample size
\jiazhi{Leskovec~\etal~\cite{Leskovec2006} show that different sampling \yuanjun{strategies} produce very similar results when the sampling rate is greater than 50\%.}
\jiazhi{Therefore, we cut off the sampled scatterplots in a sequence if their sampling rate \doc{was} greater than 50\% to avoid meaningless comparison.}
%is
%\lingyun{As it was shown in Leskovec et al.~\cite{Leskovec2006}}, different sampling techniques can produce very similar results with a sampling rate greater than 50\%, thus, we limited the number of sample points to not more than half of the original data.
%Therefore, 
As a result, there \doc{were} seven sampled scatterplots \lingyun{(at most), along with the original scatterplot with all points}, to be displayed.
\lingyun{The eight scatterplots \doc{were}} arranged in a $2 \times 4$ matrix layout, as shown in Fig.~\ref{fig:interface_1}.
%are
\revision{There were eight trials for each participant in this experiment, corresponding to eight datasets, respectively.}
It took about 5 minutes for each participant to finish the experiment.
% \yuanjun{Participants were asked which visual factors they \doc{were concerned with} in this experiment in the post-experiment questionnaire.}
\yuanjun{Participants were asked which visual factors they \doc{were concerned with} in the post-experiment questionnaire.}
% \revision{Participants were asked for the visual factors considered in this experiment in the post-experiment questionnaire.}
%in their judgments 
% \jiazhi{\textbf{TODO: add the description of subjective questionnaires.}}

\begin{figure*}[ht]
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{fig/pilot_task1_rev.pdf}
\vspace{-5mm}
\caption{Results of Experiment 1 in the pre-study (Sampling number identification). This bar chart shows the number of votes for each sampling number in each dataset. Red bars indicate the selected sampling numbers in our formal study.
% The line indicates the cumulate proportion of participants selecting the option with a sampling number not more than the current one. 
}
\vspace{-3mm}
\label{fig:pilot_task1}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fig/pilot_task2_rev.pdf}
\vspace{-5mm}
\caption{Results of Experiment 2 in the pre-study (Understanding color effect on region density identification). Q1 -- Q20 stands for the 20 generated questions. Error bars indicate 95\% confidence intervals \revision{(same as below)}. Below the x-axis listed the accuracy of each question.}
\vspace{-5mm}
\label{fig:pilot_task2}
\end{figure*}

\vspace{1mm}
\noindent\textbf{Participants and Apparatus}.
We recruited \yuanjun{160} participants (\yuanjun{130} males, \yuanjun{30} females, aged 18 -- 60 years).
% for Experiment 1.
All \doc{the} participants were either students or researchers with \doc{a} computer science background.
69 participants reported \doc{being} familiar or very familiar with visualization, 32 moderately familiar, and 61 unfamiliar or very unfamiliar.
65 participants reported previous experience with sampling.
% to be
%\lingyun{update the numbers}

\looseness=-1
%A web prototype was implemented for this experiment.
The experiment was conducted through a web prototype.
Participants were asked to perform the experiment on a screen with a resolution higher than $1,920 \times 1,080$.
% The points in the scatterplots were rendered \lingyun{with a radius of 3 pixels in random order without transparency}.
\revision{
The points in the scatterplots were rendered with a radius of 3 pixels, which was preliminarily confirmed by iterative adjustments within a common range (1--5 pixels).
Moreover, we rendered the points without transparency to avoid affecting the color perception~\cite{d1997color}.
% The radius of points was confirmed by iterative adjustings within a common range (1 -- 5 pixels) preliminarily.
% The radius of points was confirmed by iterative adjustings in a preliminary study.
% Because the sampling ratio and the radius of points affect the extent of visual clutter together, we choose to fix the radius before determing the sampling ratio.
}

\vspace{1mm}
\looseness=-1
\noindent\textbf{Results}.
Given the fact that when there are more points in \doc{a} sampled scatterplot, it will look more like the original scatterplot, \doc{we assumed that participants would consider the sampling results still similar to the original scatterplot when the sampling number was more than the selected one.}
\jiazhi{In addition, considering that other sampling strategies may perform better than random sampling, we needed to leave the space to show their superiority in our experiments.}
\lingyun{Based on these considerations, we have chosen the optimal sampling number by requiring that the sampling numbers of the scatterplots selected by 80\%, rather than 100\%, of the participants were smaller than the optimal one.}
\yuanjun{Fig.~\ref{fig:pilot_task1} presents the \lingyun{results, which shows that the optimal} sampling number for most datasets (\emph{MNIST}, \emph{Swiss Roll 2D}, \emph{Crowdsourced Mapping}, and \emph{Condition Based Maintenance}) is 2,531, while the sampling rates of them were $3.6\%$, $31.6\%$, $23.3\%$, and $25.3\%$, respectively.}
\yuanjun{Four exceptions were the datasets \emph{Clothes}, \emph{Epileptic Seizure}, \emph{Swiss Roll 3D}, and \emph{Abalone}, whose optimal sampling numbers with the corresponding sampling rates were 3,796 ($14.3\%$), 3,796 ($33.0\%$), 1,687 ($16.9\%$), and 1,125 ($26.9\%$), respectively.}
% The sampling rates of each dataset can be found in Table.~\ref{tab:outlier_ratio}.
% \lingyun{\textbf{Comments:}put the percentage}
%\lingyun{Two exceptions are the datasets \emph{Clothes} and \emph{Epileptic Seizure}, where for both the optimal sampling number was 3796 points.}
%\lingyun{\textbf{Comments:}put the percentage}.
%\lingyun{This implies that more points are needed to be sampled in a scatterplot of a higher clutter degree in order to keep the sampling result close to the original one.}
%Another exception arises in the dataset \emph{Abalone} containing only about 5000 points, while other datasets all contain more than 10000 points.
%Therefore, its proper sampling number is less correspondingly. \lingyun{check this}
\jiazhi{According to the results of the subjective questionnaire in the experiment,}
\lingyun{when judging the similarity between scatterplots, over 75\% of the participants took the overall shape of each class of points into consideration, followed by density 
($55\%$) and outliers ($35\%$).}
% (\textbf{Comments: the percentage}) and outliers (\textbf{Comments: the percentage}).}

\subsection{Experiment 2: \yuanjun{Understanding Color Effect on Region Density Identification}}

This \jiazhi{controlled} experiment aims \doc{to understand} the \lingyun{effect} of color when comparing \jiazhi{region} density \jiazhi{in multi-class scatterplots}.
%at understanding
\jiazhi{Though color is not related to the definition of region density, encoding class labels with color may affect human perception.}
%the
% \jiazhi{Therefore, although we prefer to perform the formal study \doc{with} color-encoded scatterplots rather than in single-color scatterplots, we should figure out whether color affects the perception of region density.}
\revision{Therefore, we should figure out whether color affects the perception of region density to decide whether color to be used in the formal study.}
%in
%As an irrelevant factor in the comparison of region density, color may affect the human perception.
%To figure out the perceptual effect of color helps us to decide whether we should preserve color in the experiment of comparing global density in the formal study.

% \jiazhi{\textbf{Comments: merge the Task and Experiment Design as one paragraph. Split the part of Procedure as a separate paragraph.}}

% \vspace{1mm}
% \noindent\textbf{Task and Procedure}.
\noindent\textbf{Task and Experiment design}.
\yuanjun{We generated ten synthetic datasets using mixed Gaussian distributions with 3 to 10 classes.}
%, \jiazhi{respectively}.
% we generate 10 datasets in total, some datasets may share the same number of classes.
%The datasets that we used here 
\jiazhi{These datasets} were different from the ones in the formal study.
% In each question, two rectangular regions were marked on the same scatterplot, \lingyun{and} participants were asked to compare \lingyun{\doc{the} 
% %average point 
% \jiazhi{region} density and select the region \doc{with the} higher density}.
\revision{In each question, two rectangular regions were marked on the same scatterplot, and participants were asked to select the region with the higher density.}
%which had
This experiment adopted a within-subject design, and the only variable was whether the scatterplot was colored or not.
% \lingyun{We rendered each question twice (with multiple color and with only \yuanjun{dark grey} color). 
\lingyun{We asked the same question\yuanjun{s} \yuanjun{with multiple colors or with only a dark grey color}.
\lingyun{We provided two questions} on each synthetic dataset, \yuanjun{so there were 20 different questions.}
Thus, in total, we had}
$$
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
    \yuanjun{160\ (participants)} \times 20\ (questions) \times 2\ (colors) = 6,400
$$
results.
In order to eliminate the learning effect, \yuanjun{the multi-colored and single-colored versions} of the same question were arranged \lingyun{to appear in random order and not consecutively}.
%The real test then started after a prompt page, where completion time and accuracy for each question was recorded.
%Thus, we asked the participants to finish the task as quickly and accurately as possible.
It took about 5 minutes for each participant to finish the experiment.

% \vspace{1mm}
% \noindent\textbf{Experiment Design}.
% The experiment adopted a within-subject design, and the only variable  was whether the scatterplot was colored or not.
% \lingyun{We had 20 different scatterplots and we rendered them twice (with multiple color and with only black color). We asked the same question\yuanjun{s} with both colored and uncolored scatterplots. Thus, in total, we had}
% $$
%     \yuanjun{162\ (participants)} \times 20\ (scatterplots) \times 2\ (questions) = 6480
% $$
% results.

% \vspace{1mm}
\looseness=-1
\noindent\textbf{Procedure}.
\lingyun{In order to help the participants \doc{become} familiar with the task, the experiment started with a training session of three questions.
%to get
In the training session, the correct answers were shown to the participants after they submitted their answers.
Participants could ask questions during the training session.
Time and accuracy were not recorded.
As long as the participants reported that they had fully understood the experiment, we started the real \yuanjun{test}, where completion time and accuracy for each question were recorded.
%study
Thus, in the real study, we reminded participants that they needed to finish the experiment as fast and precisely as possible.
After the experiment, participants were asked to finish a questionnaire and rate the color \lingyun{effect on} a five-point Likert scale.
}

%Thus, 20 different questions were tested in total, and each question would be asked twice, once with a colored scatterplot and once with an uncolored one.

% \vspace{1mm}
\noindent\textbf{Participants and Apparatus}.
% This part was the same as Experiment 1.
% \yuanjun{This part was the same as above.}
\lingyun{We had the same participants and used the same apparatus as in Experiment 1.}

% \vspace{1mm}
% \looseness=-1
\noindent\textbf{Results}.
% The results are shown in \yuanjun{Fig.~\ref{fig:pilot_task2}}.
\revision{As Fig.~\ref{fig:pilot_task2} shows,}
the average accuracy of the \yuanjun{multi-colored} and \yuanjun{single-colored} questions were 92.9\% and 93.3\%, respectively, while the average completion time of the \yuanjun{multi-colored} questions was \lingyun{3,581ms and \yuanjun{that} of the \yuanjun{single-colored} ones was 3,616ms}.
%\yuanjun{3616ms, which was} 235ms fewer than \yuanjun{3851ms} of the colored ones on average. \lingyun{report the actual numbers}
\yuanjun{Since the data was not subject to the normal distribution according to the Shapiro-Wilk test, we conducted \yuanjun{the} Wilcoxon test to \yuanjun{examine} the significance of their difference with \doc{a} significance level \doc{of} $\alpha = 0.05$.
%check for
No statistical significance in the difference of their accuracy is reported through \lingyun{hypothesis} tests ($p = 0.2648 > 0.05$).
But \doc{a} significant difference \doc{was shown} in terms of completion time ($p = 1.551 \times 10^{-10} < 0.001$), \revision{indicating} that participants spent significantly \doc{less} time in completing \yuanjun{single-colored} questions than multi-colored ones.}
% which means
%exists, shorter
% \lingyun{In the subjective questionnaires,
% the average score of the color deficiency was 2.03}, indicating that the participants felt that color affected the \yuanjun{region} density comparison slightly.
\revision{The subject feedback reflected that participants felt that color affected the region density comparison slightly with an average score of 2.03 of the color deficiency.}
This is also \doc{consistent} with our numerical results.
%coherent
A participant commented that \emph{"the salient color may have an influence on my judgment of density."}
Consequently, we decided to \yuanjun{use single-colored scatterplots} in the experiment of \yuanjun{region} density comparison in the formal study to eliminate the color effect.
%remove color

% \begin{table}[t]
% \centering
% \caption{Result of Experiment 2 in the pre-study: Color effect on all-class density comparison}
% \begin{tabular}{c|cc}
% \toprule
% & Accuracy & Completion time \\
% \midrule
% Colored & 92.9\% & 3616ms \\
% Uncolored & 93.3\% & 3851ms \\
% \bottomrule
% \end{tabular}
% \label{tab:pilot_task2}
% \vspace{-3mm}
% \end{table}


==> Evaluation of Sampling Methods archive/5-experiments.tex <==

\section{Formal Study}
%\section{Preliminaries}
\label{sec:experiments}
%The formal study aims to evaluate the performance of selected sampling strategies in the aspects of maintaining three identified visual factors, including density, outlier, and overall shape.

\subsection{Hypotheses}
% define the hypotheses here.
%\yuanjun{TODO: raise the hypothesis in the first sentence}
%We raise the following hypotheses according to the three aspects to be evaluated in our experiments.
\looseness=-1
\doc{This} formal study aims to evaluate the performance of seven selected sampling strategies \doc{based on} preserving three identified visual factors, including relative density, outlier, and overall shape.
%The, in the aspects of
According to the three visual factors, we \doc{formulated} four hypotheses to guide the experiment design.
Specifically, we \doc{formulated} two hypotheses on relative density in terms of \emph{region density} and \emph{class density}, respectively.
\emph{Region density} refers to the density of data points regardless of class information.
\emph{Class density} is the density of data points belonging to a certain class.

% \vspace{1mm}
\noindent\textbf{H1:}
% RS will perform better in terms of completion time in the two experiments about relative density.
% We propose this hypothesis because the proportion of points between different regions or different classes in the sampling results of RS will be consistent with that of the original data in the statistical sense.
% As color will disturb the perception on density to some extent, we also assume that the completion time of Experiment 2 will longer than that of Experiment 1.
% Besides, we believe that the accuracy between different sampling methods will be little, since none of them will reverse the density relationships in their sampling results.
\textbf{All other sampling strategies perform better than random sampling in preserving relative region density.}\\
%relative density identification tasks.}
Maintaining relative density is a common goal for many sampling strategies~\cite{Chen14, Chen20, Hu20}. Compared to random sampling, these strategies are designed with delicate algorithms.
They often report positive results when \doc{compared} with random sampling in different scenarios~\cite{Chen20}.
Therefore, we assume all other sampling strategies should perform better than random sampling in preserving relative region density.
%comparing

% \vspace{1mm}
\noindent\textbf{H2: Multi-class adapted sampling strategies perform better than other sampling strategies in preserving relative class density.}\\
Many sampling strategies \doc{are customized for multi-class scatterplots.}
%the scenario of
In these strategies, preserving the individual class properties, \eg, density, is an important goal.
Therefore, we assume that multi-class adapted sampling strategies, including multi-view Z-order sampling~\cite{Hu20}, recursive subdivision based sampling~\cite{Chen20}, and multi-class blue noise sampling~\cite{Chen14}, perform better than the other four sampling strategies in preserving relative class density.

%As RS is the baseline method, we believe that all other sampling methods are well-designed so that they should perform better than RS in the two experiments about relative density.

% \vspace{1mm}
\noindent\textbf{H3:}
\looseness=-1
\textbf{Outlier biased density based sampling is the best in preserving outliers.}\\
%the outlier identification task.}
Many sampling strategies have shown \doc{an} ability \doc{to preserve} outliers in their reports. Among them, outlier biased density based sampling is designed especially for preserving outliers. It is the only strategy that integrates outlier measures into the sampling process. Therefore, we assume that outlier biased density based sampling is the best strategy \doc{for} preserving outliers.
%their, in preserving, in

%Outlier biased density based sampling is designed to preserve more outliers from the original data specifically.
%Although some other sampling methods also show their ability to preserve outliers in their sampling results, we still consider outlier biased density based sampling as the best in outlier maintenance.

% blue noise sampling regular points
% BNS will obtain relatively higher precision in identifying outliers for the reason that the distances between normal points in their sampling results will be more uniform, which makes it easier to highlight outliers with abnormal distances to the main distribution or with abnormal classes from their neighboring points.
% BNS and MCBNS will obtain relatively higher precision in identifying outliers for the reason that they will produce sampling results with more evenly distributed points, which is beneficial for people to tell the class difference and distance difference of a point.
% On the other hand, OBDBS and RSBS will outperform other sampling methods in the recall of outliers because they tend to sample more outliers in the sampling process.

% \vspace{1mm}
\noindent\textbf{H4:}
\textbf{Blue noise sampling \yuanjun{and multi-class blue noise sampling perform} better than other strategies in preserving the overall shape.}\\
In our observation, uniform distribution facilitates the description of shapes by minimizing the effects of other visual factors, such as outliers and inhomogeneous density.
Based on \doc{this} observation, we assume that \yuanjun{sampling strategies that aim to generate uniform samples with blue noise property, \yuanjun{\ie}, blue noise sampling and multi-class blue noise sampling}, should perform the best in preserving the overall shape.
%the
%we assume that a more even distribution of sampled points will be beneficial to preserving their overall shapes.
%Based on such assumption, we hypothesize that BNS will achieve better results than other sampling methods since it can produce sampled points with blue noise properties, which make them distribute more evenly.
% We believe that sampling methods that can sample more points at the boundary of each class will better preserve the overall shapes in the original scatterplots.
% Therefore, BNS, MCBNS, OBDBS, RSBS will perform better than RS, DBS, MVZS.
% Another consideration is that more evenly distribute points will help people recognize the overall shapes, so BNS will outperform other sampling methods from this perspective.


%\subsection{Participants and Apparatus}
%Participants, Stimuli, and Apparatus}
% 2 groups of people: 20 Visualization knowledgeable and 20 Machine learning knowledgeable. When collecting data, there should be more than 20 people in each group to remove outliers in our results. (Before)
% \vspace{1mm}
%\noindent\textbf{Participants}.
%We recruited 101 participants (78 males, 23 females, aged 18-50 years, \lingyun{average?} \yuanjun{we just ask for their age range}) for the formal user study.
%All of them reported no color vision problems.
%Sixteen of them are researchers, while others are students majoring in computer science.
%Thirty-four participants reported previous experience with sampling.
%Each participant was rewarded 160 RMB for completing the experiments.
% How many people attended the study? Background: gender, age, major, whether familiar with scatterplots or sampling, color blindness or color weakness problems
% Rewards to the participants

%\vspace{1mm}
%\noindent\textbf{Apparatus}.
%A web prototype was implemented for the formal user study \jiazhi{(see Figure xxx)}.
%Participants were required to visit it remotely on the Chrome browser and finish the experiment on a screen with a resolution of $1920 \times 1080$.
%They were asked to share their screens with us during the experiments, \yuanjun{
%so that we can monitor their behaviours in the training sessions to ensure that they fully understand our tasks before the actual test.}
%\yuanjun{Moreover, in case they encounter any questions during the test such as disconnection to our server, they can also present them on their screen and ask for our help.}
%\lingyun{report if it happened in the study}
%The points in the scatterplots were rendered in a random order \lingyun{It matters? \yuanjun{To prevent a class of points to be totally overlap by other ones}} with a radius of 3 pixels and without transparency.

% \paragraph{something else}

%\vspace{1mm}
%\noindent\textbf{Testing data}.
%Based on the results in the preliminary study, each dataset \lingyun{were} sampled to certain number of points.
% would be
%For the sampling methods which are not able to sample an exact number of points (MVZS, RSBS), we adopted the sampling results %with less than 1\% sampling number error.
%To guarantee fairness, the sampling results displayed to each participant were produced by the same random seeds.
%The questions in the actual tests were designed based on the sampling results. \lingyun{of the pre-study?}


% The selection and argumentation of data.
% 1) Use Scagnostics to select datasets that cover different aspects.(jiazhi)

% Here talk about the pilot study if you want, because it is related to the dataset chosen.

% \textbf{Pilot Study}
% 1) To estimate the lasting time of our user study

% 2) Help to choose datasets:
%     2.1) Remove datasets with similar results
%     2.2) Remove datasets with too much time cost

% (3) determine the sampling rate

% (4) determine the experimental order

\subsection{Experiments}
% define the tasks here.

% 1) Summarized from existing literature.

% 2) *** Each task need to be specified what it learns (the hypothesis, the conclusion, what the users focus on, etc.)

% 3) Tasks should be in a simple form in order to ease the burden of the participants.

% 4) How to determine ground truth patterns. With severe overdrawing problems, it may not be accurate on the original scatterplot. (jiazhi)

% 5) How to determine outliers: majority voting using sklearn algorithms. (shixia)

% 6) The research of interest on single class sampling: density, outliers, shape.
% When extended to multi class sampling: study effects of both single class and overall

% 7) Can people separate the perception of density and shape?

% 8) Task 3: Identify outliers?

% First, we identified the most critical factors for the sampling methods.
% We extracted the \emph{design requirements} and the \emph{application goals} \lingyun{make sure these two phrases} of the sampling methods from our survey.
% As visual clutter reduction is common in sampling, we did not take it into consideration. \lingyun{not very convincing, because it is common, so we did not take into consideration?}
% \textbf{Outlier maintenance} was the most mentioned, which appeared in seven papers \yuanjun{out of the 26 papers}.
% Moreover, three and two of the papers also concerned about preserving \textbf{relative density} and \textbf{overall shape} of the scatterplots, respectively.
% \lingyun{did you mention how many papers in total?} \yuanjun{Yes, in section 3.1.1, now also mentioned above}
% Given such results,

%Based on the visual factors identified in Sec.~\ref{sec:factor}, we \yuanjun{concluded} the tasks related to these subjects from scatterplots evaluations~\cite{Chen14, Hu20, Zhao2019} and designed our experiments based on them.
% \lingyun{consulted?}
%Experiments 1 - 3 are controlled experiments, while Experiments 1 and 2 are related to relative density preservation, and Experiment 3 is related to outlier maintenance.
%Experiment 4 is a subjective experiment related to overall shape preservation.
% \looseness=-1
Guided by the four hypotheses (\textbf{H1}--\textbf{H4}), we designed four experiments:
Experiment 1 (\textbf{E1}) was designed for the perception of relative region density preservation (\textbf{H1}), and Experiment 2 (\textbf{E2}) was designed for the perception of relative class density preservation (\textbf{H2});
Experiment 3 (\textbf{E3}) was designed for the perception of outlier maintenance (\textbf{H3});
Experiment 4 (\textbf{E4}) was for the perception of overall shape preservation (\textbf{H4}).
Note that \textbf{E1}--\textbf{E3} \doc{were} controlled experiments, and \textbf{E4} \doc{was} a subjective experiment.

\begin{figure}[!b]
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{fig/interface_E1.pdf}
\vspace{-5mm}
\caption{Example interface of \textbf{E1} in the formal study.}
\vspace{-5mm}
\label{fig:interface_E1}
\end{figure}


% introduce the experiment, what to test - why - how
% \vspace{1mm}
\noindent\textbf{E1: Perception of relative \yuanjun{region} density preservation}.
This experiment was used to evaluate the ability of different sampling strategies \doc{to preserve} relative region density in the aspect of visual perception.
%in preserving
%Specifically, given two regions in a scatterplot, this experiment aimed to test if the region of higher all-class density is still perceived as having higher all-class density after sampling.
Specifically, in \doc{this} experiment, we aimed to test if the region with higher \yuanjun{region} density can still be recognized as the higher one after sampling.
% the
Thus, in each question, we randomly marked out two rectangle regions with the size of $\frac{w}{5}\times\frac{w}{5}$, where $w$ is the width of scatterplots.
Participants were asked to select the region with \doc{a} higher density \yuanjun{without considering class labels}.

%\jiazhi{Participants were asked to select the region with higher average point density than the other.}
Based on the result of the pre-study, color would interfere and slow down the judgments of the participants.
Thus, we rendered all data points in dark grey regardless of their labels.
We had eight datasets, and we generated two questions for each dataset.
For each question, we generated seven trials corresponding to seven sampling strategies, respectively.
In the seven trials of the same question, the locations of the rectangle regions were the same.
In total, we had
$$
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
    7\ (sampling\ strategies) \times 8\ (datasets) \times 2\ (questions) = 112
$$
trials for each participant.

%\jiazhi{For each dataset, we generated two series of trials by selecting two different region pairs, respectively.}
%\jiazhi{Each series contained seven trials, which are created by seven sampling strategies on the same dataset, respectively.}
%\jiazhi{Eight dataset, two series, and seven sampling strategies resulted in $112$ trials for each participant.}

%\noindent\textbf{Experiment 1: Perception on \yuanjun{relative all-class density}.}
%This experiment was designed to compare the ability of different sampling methods to preserve \lingyun{in preserving} human perception on global density.
%In each question, we provided the scatterplot of a specific sampling result and marked out two regions \yuanjun{of the same size ($\frac{1}{5} \text{width} \times \frac{1}{5}\text{height of the scatterplot}$)}
% \lingyun{size, give actually number?}.
%Participants were asked to select the region with higher average point density.
%As demonstrated in the preliminary study, color could interfere and slow down the judgments of the participants, so we remove color in the scatterplots in the experiment.
%We generated two questions on each dataset.
%Thus, the total number of questions for each participant were:
%\lingyun{usually we talk about how many results do we get here.}
%Thus, the total number of results we got in the experiment is
%$$
%    \yuanjun{101\ (participants)} \times 7\ (sampling\ methods) \times 8\ (datasets) \times 2 = 11312.
%$$
%Completion time and accuracy for each question were recorded.

% \vspace{1mm}
\noindent\textbf{E2: Perception of relative \yuanjun{class} density preservation.}
This experiment was used to test whether the class \doc{with} a higher density can still be recognized as the higher one after sampling.
%\jiazhi{This experiment tested whether the class have higher density than another class is still perceived as the one with higher density after sampling.}
In contrast to \textbf{E1}, \textbf{E2} focuses on preserving relative density of specific classes \yuanjun{in the same region} instead of relative \yuanjun{region} density.
Thus, the scatterplots are rendered using color to encode class labels.
Specifically, in each question, we marked out a rectangle region with the size of $\frac{w}{5}\times\frac{w}{5}$ in a scatterplot.
We specified two classes in the question, and the participants were asked to choose the class with higher average density in the marked region.
\revision{In order to ensure fairness, the color assigned to each class in a specific dataset was identical across all sampling strategies.}
Similar to \textbf{E1}, we generated two questions for each dataset and seven trials for each question. In total, we had
% $7 \times 8 \times 2 = 112$
$$
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
    7\ (sampling\ strategies) \times 8\ (datasets) \times 2\ (questions) = 112
$$
trials for each participant.\looseness=-1

%\jiazhi{For each dataset, we created two series of trials with two different regions, respectively.}
%\jiazhi{Each series contained seven trials by seven sampling strategies, respectively.}
%\jiazhi{Similar to \textbf{E1}, we created $7 \times 8 \times 2 = 112$ trials for each participant.}

%\noindent\textbf{Experiment 2: Perception on \yuanjun{relative per-class density}.}
%This experiment was designed to compare the ability of different sampling methods to preserve \lingyun{in preserving} human perception on per-class density in a local region.
%In each question, we also provided the scatterplot of a specific sampling result, where colors encode class labels of the points, with a region marked out.
%Two options of classes were given, and participants were asked to select the one with higher average point density in the marked region.
%Similar to Experiment 1, we generated two questions on each dataset, \yuanjun{so we also obtained 11312 results of the questions in this experiment.}
% \lingyun{same problem here}

% \vspace{1mm}
\noindent\textbf{E3: Perception of outlier maintenance.}
This experiment was used to evaluate the ability of sampling strategies in preserving outliers in the aspect of perception.
We tested: (1) whether an outlier in the original dataset can still be preserved and perceived as an outlier after sampling; and (2) in case a point is perceived as an outlier after sampling, whether it is indeed an outlier in the original dataset.

%the points that are of different classes with its neighboring points; the points that are far from the main distribution areas.

%\jiazhi{We tested: (1) whether an outlier is preserved and perceived as outlier after sampling; and (2) whether a point was an outlier if it is perceived as an outlier after sampling.}

There are diverse definitions of outliers, however, here we focused on the outliers in two \doc{situations}: first, when considering class labels, the point that is of \doc{a} different class \doc{from} its neighboring points; second, when not considering class labels, the points which are located \yuanjun{at abnormal distances} from its class.
%scenarios
% far away
We followed the definition in the class purity algorithm~\cite{Motta2015} in the first scenario and followed the local outlier factor algorithm ~\cite{pedregosa2011scikit} in the second scenario.

%\jiazhi{The definition of outlier would be diverse.}
%\jiazhi{We focused on two scenarios.}
%\jiazhi{When considering class labels, the point that is of different class with its neighboring points is defined as outliers.}
%\jiazhi{Specifically, we followed the definition in the class purity algorithm [Cite here]).}
%\jiazhi{Regardless of class labels, we defined the outlier by the local outlier factor algorithm~\cite{pedregosa2011scikit}.}
\looseness=-1
\yuanjun{In each question, we marked out a region in a scatterplot.}
Participants were asked to mark the outliers \doc{assuming} they \doc{believed} the outliers existed in the marked region.
%in case, judge
% with the size of $\frac{w}{5}\times\frac{w}{5}$
% Here the size of the rect region depends on how many outliers are in the datasets.
Note that, the outliers were referring to all points in the entire scatterplot, instead of the marked region.
We \doc{considered} three ways for participants to identify outliers:
%had
first, marking out all the outliers in the entire scatterplot;
second, marking out a specified number of outliers (\eg, 10) in the entire scatterplot;
and third, marking out all outliers in a given rectangle region.
Considering the huge \doc{number} of outliers in the entire dataset, it is not feasible to mark all \doc{of them} in the entire range in the limited experiment time.
%size
%out
\doc{In addition}, the accuracy would be very low since \doc{many} outliers would be missed.
% Besides, a lot of
If we limit the number of target outliers as noted in the second option, due to the large number of outliers, participants may easily mark \doc{the} requested number of outliers.
%out all
The accuracy would be high for all \doc{the} strategies, and it would be hard to distinguish the performances of different sampling strategies,
% So that
\doc{so} we chose the third option and asked the participants to mark all the outliers in a fixed range.
%finally
%out
The only disadvantage \doc{with} this option was that participants might mis-select outliers referring to the local distribution.
% of
To avoid this, we reminded the participants to refer to global distribution, and we also corrected the observed errors in the training session.
In total, we had
$$
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
    7\ (sampling\ strategies) \times 8\ (datasets) = 56
$$
trials for each participant in this experiment.

%\jiazhi{Participants were asked to identify whether outliers existed in the marked region referring to all points in the entire scatterplot and mark the outliers if they reported yes.}
%below is not a very good reason
%\jiazhi{Because marking outliers is time consuming, we created only one series of trials by specifying a region for each dataset to make sure that the experiments can be completed in a reasonable time.}
%\jiazhi{Each series contained seven trials by seven sampling strategies, respectively.}
%\jiazhi{Therefore, we created $7 \times 8 = 56$ trials for each participant.}


%\noindent\textbf{Experiment 3: Perception on outlier maintenance.}
%As for measuring the ability to maintain outliers of the sampling methods, it contains two aspects: (1) A good sampling method should preserve as many outliers as possible, and (2) outliers can be correctly perceived by the human in the sampling result.
%Thus, in this experiment, we aimed at figuring out which sampling methods could help people better perceive on outliers.
%The definition of outliers could be \lingyun{diverse}, but only two usual kinds of outliers were included in this experiment: the points that are of different classes with its neighboring points; the points that are far from the main distribution areas.
% kaleidoscopic
%\lingyun{do you need to explain the reasons that we only include these two kinds of outliers?}
% How to determine outliers: majority voting using sklearn algorithms. (Discussed in Chapter 6?)
%We marked out one region on each scatterplot of the sampling results, and the region would be exactly the same for the same dataset. \lingyun{not clear}
%Participants were asked to identify whether outliers existed in the region of the scatterplot referring to the global distribution, and mark them out if yes.
%Since identifying outliers is a somewhat \lingyun{remove somewhat?} subjective behavior, the participants were required to hold a similar principle during the experiment.
%Totally, the number of results in this experiment were:
%$$
%    \yuanjun{101\ (participants)} \times 7\ (sampling\ methods) \times 8\ (datasets) = 5656.
%$$
%\lingyun{* participants number}
%The points chosen in each sampling result were recorded.

\looseness=-1
% \vspace{1mm}
\noindent\textbf{E4: Perception of overall shape preservation.}
This experiment was used to compare the abilities of sampling strategies \doc{to preserve} the overall shape of scatterplots in terms of visual perception.
% in preserving
In contrast to \textbf{E1}--\textbf{E3}, \textbf{E4} was a subjective experiment.
In each trial, we sampled a dataset using seven strategies and displayed these seven sampling results together with the original scatterplot (see Fig.~\ref{fig:interface_1}).
Participants were asked to rank the seven sampling results based on the shape similarities between the sampling results and the original scatterplot.
Participants were reminded that class labels should be taken into account in comparing the shape similarities.
%\noindent\textbf{Experiment 4: Perception on overall shape preservation.}
%This experiment aimed at figuring out which sampling methods could preserve the overall shapes of the original scatterplots in terms of human perception.
%For each dataset, we displayed its original scatterplot along with the sampling results of the seven evaluated sampling methods in a $2 \times 4$ matrix layout like Fig.~\ref{fig:interface_1}.
%Participants were asked to rank the sampling results based on the similarity of overall shapes of each class of points compared with the original scatterplot.
Parallel rankings were allowed when participants could not distinguish the difference among the sampling results.
% In total, each participant had eight trials for the eight datasets in this experiment.
\revision{Each participant had one trial for each dataset.
Thus, in total, we had eight trials for each participant in this experiment.}
%There are eight questions \yuanjun{for each participant} in this experiment, which was equal to the number of the selected datasets.
%\yuanjun{We got
%$$
% \yuanjun{101\ (participants)} \times 8\ (datasets) = 808
%$$
%ranking results in this experiment.}
%\lingyun{give the total number of results like before}
%\jiazhi{The eight dataset resulted in eight trials for each participant.}

%Since we have eight datasets, in this experiment we had eight trials for each participant.

\subsection{Participants, Apparatus and Testing Data}

\noindent\textbf{Participants}.
We recruited 100 participants (78 males, 22 females, aged 18--50 years, average: 24) for the formal study.
%All of them were with normal or corrected-to-normal vision.
16 of them are researchers in visualization and computer graphics.
The others are undergraduates or graduated students majoring in computer science.
34 participants reported previous experience with sampling.
None of them reported color blindness or color weakness.
Each participant was rewarded \$20 per hour for completing the experiments.

\noindent\textbf{Apparatus}.
% The experiments were conducted online, and a web prototype was implemented for the formal user study (see Figure \ref{fig:interface_3}).
\revision{The experiments were conducted online through a web prototype (see Figure \ref{fig:interface_E1}).}
Participants were required to visit it remotely on the Chrome browser and finish the experiment on a screen with a resolution of $1,920 \times 1,080$.
They were asked to share their screen with the instructor during the experiments to enable remote monitoring.

% \looseness=-1
\noindent\textbf{Testing data}.
We generated scatterplots based on the \doc{eight selected} datasets for the experiments \revision{in advance}.
For each dataset, we created one scatterplot of the original dataset and seven scatterplots of sampling results by the seven sampling strategies, respectively.
The sampling rates of each dataset were determined \doc{based on} the results of the pre-study.
% by
Since multi-view Z-order sampling and recursive subdivision based sampling cannot set the exact sampling rate, we controlled the error \doc{at} $1\%$.
%in
\yuanjun{The points were rendered with a radius of 3 pixels without transparency.
The size of the scatterplots was $1,000 \times 1,000$ pixels in \textbf{E1}--\textbf{E3}, and $300 \times 300$ pixels in \textbf{E4}.}
In order to avoid imbalanced occlusion between classes, the points in the scatterplots were rendered in random order.
Except for \textbf{E1}, we selected Boynton's color palette~\cite{Boynton1989} to encode classes in the scatterplots.
%\yuanjun{To help people recognize different classes of points in the multi-class scatterplots, we selected the colors for encoding classes based on a palette with colors that are hard to be confused~\cite{Boynton1989}.}
% All scatterplots were generated in advance.
%and provided to all participants.
For the training session, we generated synthetic datasets following the Gaussian mixed distribution.
In the real testing session, the order of all \doc{the} questions was counterbalanced by following a Latin square to avoid the learning effect.

%\noindent\textbf{The order of trials}.\lingyun{remove "The order of trials"?} The only experiment variable in \textbf{E1}--\textbf{E3} was the sampling strategy. Thus, in order to avoid the learning effect, the order of all questions were arranged and counterbalanced by following a Latin square.

%\noindent\textbf{The order of trials}.
%\jiazhi{For experiments \textbf{E1}--\textbf{E3}, we carefully designed the order of trials.}
%\jiazhi{In our within-subjects design of the three controlled experiments, the variable was the sampling strategy.}
%\jiazhi{A participant answered the same question for seven times with different sampling strategies.}
%\jiazhi{Learning effects occurred in the test. }
%\jiazhi{Therefore, the order of trials presented to each participant were counterbalanced following Latin squares in order to reduce the learning effect.}

%\subsection{Experiment design}
%For the controlled experiments, we adopted a within-subjects design.
%The variable in the experiments is the sampling method.
%That meant the participants would meet similar questions during their test, which corresponded to the same dataset but with different sampling methods.
%Therefore, the order of datasets and sampling methods displayed to each participant would be counterbalanced following Latin squares in order to reduce the learning effect.

%\noindent\textbf{User interaction}.
%\noindent\textbf{\jiazhi{The interactions for identifying outliers}}.
%\lingyun{say a few words about user interactions in other experiments}
%When designing \textbf{E3}, we have considered three ways for participants identifying outliers:
%\lingyun{explain why it is important to design user interaction for identifying outliers}
%first, marking out all the outliers in the entire scatterplot;
%second, marking out a specified number of outliers (e.g., 10) in the entire scatterplot;
%and third, marking out all outliers in a given rectangle region.

%Considering the huge size of outliers in the entire dataset, it is not feasible to mark all out in the entire range in the limited experiment time. Besides, a lot of outliers would be missed. Even if we limit the number of outliers, participants would still spend too much time to search them in the entire range.
%However, our goal was to test if participants were able to recognize the outliers from the sampled scatterplots precisely and quickly.
%Thus, we final chose the third option and asked the participants to mark all the outliers in a fixed range as precisely and quickly as possible.
%\jiazhi{However, because there would be several hundreds of outliers, it is not feasible to mark out them all in an experiment.}
%\jiazhi{The second option is to mark out a specified number of outliers (e.g., 10) in the entire scatterplot to make the experiment feasible.}
%\jiazhi{Considering the possible big number of outliers, the accuracy would be high for all the answers.}
%\jiazhi{It would be hard to distinguish the performances of different sampling strategies.}
%\jiazhi{The third option is to the one we chose.}
%\jiazhi{The participants were given a rectangle region and asked to mark out all outliers in the region.}
%The only disadvantage of this option was that participants might be misled to select outliers referring to the local distribution.
%To avoid this, we reminded the participants to refer to global distribution and correct the observed errors in the training session.

%We have considered several options for identifying outliers referring to the global distribution in Experiment 3.
%One is to ask participants to mark out all the outliers in the whole scatterplot of the sampling results, but it was too time-consuming.
%Another option is to ask them to mark out a certain amount of points (e.g., 10) that they considered most likely to be outliers in the whole scatterplot.
%It was hard to distinguish the performance difference among the sampling methods nevertheless.
%Finally, we decided to take the current design that we ask participants to mark out outliers in the given region of the scatterplot, which could address the time-consuming problem to a certain degree.
%It was the most feasible way despite that it might be somehow misleading that participants might refer to the local distribution of the given region.
%To reduce such negative effect, we will repeatedly remind the participants in the training session of this experiment that they should refer to the global distribution when judging whether a point is an outlier.

\subsection{Procedure}

Each experiment included a training session and a real test session.
At the beginning of the training session, the instructor explained the experiments as well as the related concepts (\eg, outliers).
%and introduced the procedures to the participants.
After the explanation, several practice trials (three for \textbf{E1}--\textbf{E3}, and one for \yuanjun{\textbf{E4}}) were presented to help participants get familiar with the experiments.
For controlled experiments, \textbf{E1}--\textbf{E3}, the correct answers were shown to the participants after the answers were submitted.
%Next, several demo questions same as in actual tests with different datasets will be presented.
%The instructor introduced the system interface and the interactions to the participants, and then they practised with the demo questions in order to get accustomed to the system and the tasks.
%They are
The participants were encouraged to ask questions in the training sessions to facilitate their understanding of the experiments.
After they reported that they have fully understood the tasks, we started the real test session.
Participants were allowed to have a break of five minutes before each experiment.
%until they fully understood the experiments.
%A prompt page would be shown as notice before the actual tests began.
%Four
%\jiazhi{Three} breaks
%were provided to the participants between each experiment
%\jiazhi{between every two experiments}
%and
%\jiazhi{one breaks }
%in the middle of Experiment 3
%\jiazhi{were provided to the participants}.
%\jiazhi{Each break lasted five minutes.}
After the participants completed all the experiments, they were asked to
answer a questionnaire for their backgrounds and subjective feedback on the experiments.
The entire process lasted approximately one hour and 20 minutes for each participant.

% \vspace{1mm}
\looseness=-1
The questionnaire included three parts.
First, we asked participants \doc{about their} backgrounds and basic information, familiarity with visualization, and experience with sampling strategies.
Second, participants were asked to rate the importance of
preserving relative density, outliers, and overall shape for a sampling strategy using a five-point Likert scale.
%a sampling method's ability in preserving relative density, outliers, and overall shapes
% They were also encouraged to offer any ideas about the ability a sampling method should own.
They were also encouraged to add extra abilities that a sampling method should provide.
\doc{Finally}, we asked \doc{about} their focus in each experiment in order to learn the important visual factors for human perception.
%At last
% we asked for them which factors they would focus on during each experiment for the purpose of finding out the important visual factors for human perception.

% Before the actual experiment, we introduced ... Participant were practiced with (how many) additional training datasets to get accustomed to the tasks...

% \textit{Training section}
% 1) Use questions the same as in formal tests, but different datasets.

% \textit{Real testing}

% \textbf{Experiment 1}
% introduce the experiment, what to test - why - how

% \textbf{Experiment 2}

% \textbf{Experiment 3}

% \textbf{Experiment 4}

% In the end of the study, participants were asked to finish a questionnaire.

% 1) Include background investigation, subjective questions(removed, use side-by-side comparison). Can be done afterwards in paper form.

% Time: approximately 1h preferred, and not more than 1.5h

% 3) learning effect: when performing the same task, participants may perform better as time goes by.
%     3.1) Repeated tasks, but it will take longer time.
%     3.2) Use a Latin square to order the sampling methods presented to participants).

% 4) Random sampling can be regarded as a baseline method

% 5) Which sampling rate would be appropriate? *Experiment on numerical measures

% 6) Be organized according to tasks (lingyun)

\begin{figure}[!b]
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{fig/formal_task1_new.pdf}
\vspace{-6mm}
\caption{Average accuracy and completion time of \textbf{E1} (Perception of relative region density preservation).
% \vspace{-7mm}
% Error bars represent 95\% confidence intervals.
}
\label{fig:formal_task1}
\end{figure}

==> Evaluation of Sampling Methods archive/6-results.tex <==
\section{Experimental Results}
\label{sec:results}

% 1) The amount of our data should be reported to improve the credibility of our statistical methods.

%\noindent\textbf{Measurements.}
%\noindent\textbf{Experimental records.}
\subsection{Analysis Approach}
We recorded the objective measurements from \textbf{E1}--\textbf{E3} and the subjective measurement from \textbf{E4}.
For \textbf{E1} and \textbf{E2}, we recorded the correctness and completion time of each trial.
For \textbf{E3}, we calculated the precision and recall of each trial.
In each trial, we denoted the set of outliers marked out by a participant as $M$ and the ground truth as $N$.
The precision is the ratio of $|N \cap M|$ \jiazhi{to} $|M|$, and the recall is the ratio of $|N \cap M|$ \jiazhi{to} $|N|$, where $| \cdot |$ denotes to the cardinality of a finite set.
Note that the recall refers to the ratio of outliers that are preserved by sampling and then perceived by participants.
To avoid small values, we normalized the recall by the maximal outlier preserving ratio among seven sampling strategies on each dataset.
Without \yuanjun{loss} of clarity, we use the term \emph{recall} to refer to normalized recall in the rest of this paper.
For \textbf{E4}, we recorded the ranking of each sampling strategy in each trial and \doc{transformed} the rankings into scores.
%transferred
Specifically, the 1st--7th sampling strategies get 7--1 point, respectively.

%\textbf{E1} -- \textbf{E3} are controlled experiments, where we mainly analyze their objective results.
%For \textbf{E1} and \textbf{E2}, accuracy and average completion time of each question will be calculated, while for \textbf{E3}, the precision and recall of outliers marked out by the participants will be calculated.
%Here, let $N$ is the set of outliers in the ground truth, and $M$ is the set of outliers marked out by participants.
%Prescision is the ratio of $|N \cap M|$ and $|M|$, and recall is the ratio of $|N \cap M|$ and $|N|$, where $| \cdot |$ denotes to the cardinality of a finite set.
%Furthermore, recall is normalized by the maximal retention ratio of outliers in the sampling results for each dataset.
%For \textbf{E4}, we compute the average rating scores of the sampling methods on all or on each dataset.
%For each trial, the sampling method which ranks the first gets 7 points; the second gets 6 points, and so on.
%The scores of the sampling methods that share a parallel ranking are the   average of their original scores.
%For example, if rankings $2, 3, 4, 5$ are tied, each of them will get $(6 + 5 + 4 + 3) / 4 = 4.5$ points.

\looseness=-1
Following the common \doc{methods for} evaluating user performance~\cite{lam2012empirical}, we reported the mean values and confidence intervals of the objective measurements and performed significance analyses to test our hypotheses.
% means in
For the results of \textbf{E1}--\textbf{E3}, we performed \doc{the} Shapiro-Wilk test and found that they do not follow the normal distribution.
Therefore, we employed a non-parametric method to examine whether significant differences exist among the sampling strategies.
Specifically, we chose the Friedman test with the standard significance level \doc{of} $\alpha = 0.05$ in our analysis.
If there \doc{were} significant differences, we conducted \doc{the} Conover test as the post-hoc test to examine the pairwise significance.
%The null hypothesis of each test it that the two sampling strategies perform the same.
In \textbf{E4}, we also reported the mean value and the confidence interval of the rating score for each sampling strategy.

\begin{figure}[!b]
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{fig/DAG_task1_acc_rev.pdf}
\vspace{-8mm}
\caption{Graphical depiction of the pairwise significance relationships of the accuracy differences of the sampling strategies in \textbf{E1}. A directed edge indicates that the origin sampling strategy performs significantly better than the destination one. Same as below.}
% \vspace{-7mm}
\label{fig:DAG_task1_acc}
\end{figure}

\begin{figure}[!b]
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{fig/DAG_task1_time_rev.pdf}
\vspace{-8mm}
\caption{Graphical depiction of the pairwise significance relationships of the completion time differences of the sampling strategies in \textbf{E1}.}
% \vspace{-5mm}
\label{fig:DAG_task1_time}
\end{figure}

%\noindent\textbf{Significance analysis.}
%Following the common means in evaluating user performance~\cite{lam2012empirical}, in \textbf{E1} -- \textbf{E3}, we give out the mean as well as the confidence interval of the objective measures and perform significance analysis on them.
%First, we examine the normality of the differences of each objective measure of each sampling strategy pair.
%According to the Shapiro-Wilk test, they do not always obey the normal distribution, so we use non-parameter tests with standard significance level $\alpha = 0.05$ are in the following analysis process.
%Then a Friedman test will be conduceted to examine whether significant differences exist in the objective measures of the sampling strategies.
%If yes, for each pair of sampling methods, we will conduct Conover tests as our post-hoc tests to examine the pairwise significance.
%The null hypothesis of each test is always that the sampling strategies perform the same.
%In \textbf{E4}, we also give out the mean as well as the confidence interval of the rating scores for each dataset and the union to explore whether such rating scores are consistent on all datasets or depend on the characterisitcs of the datasets.

% Here, the ground truth of the outliers consists of the points given by the local outlier factor algorithm~\cite{pedregosa2011scikit} and those that do not share the same class label with their nearest neighbors.
% % scikit-learn
% Similar to the previous experiments, we will also give the mean and the confidence interval of the precision and recall, and do the significance analysis as above.

% \begin{table*}[h]
% \centering
% \caption{Result of Experiment 1 in the formal study: Perception on all-class density}
% \begin{tabular}{c|ccccccc}
% \toprule
% Sampling method & RS & BNS & DBS & MVZS & MCBNS & OBDBS & RSBS \\
% \midrule
% Accuracy & 98.6\% & 98.4\% & 97.3\% & 96.5\% & 94.6\% & 95.0\% & 95.2\% \\
% Completion time (ms) & 2855 $\pm$ 74 & 3016 $\pm$ 89 & 2939 $\pm$ 79 & 3038 $\pm$ 92 & 3283 $\pm$ 116 & 3062 $\pm$ 90 & 3234 $\pm$ 122 \\
% \bottomrule
% \end{tabular}
% \label{tab:formal_task1}
% % \vspace{-3mm}
% \end{table*}

% \begin{table*}[h]
% \centering
% \caption{Result of Experiment 2 in the formal study: Perception on per-class density}
% \begin{tabular}{c|ccccccc}
% \toprule
% Sampling method & RS & BNS & DBS & MVZS & MCBNS & OBDBS & RSBS \\
% \midrule
% Accuracy & 90.3\% & 93.1\% & 89.7\% & 92.2\% & 92.1\% & 90.3\% & 93.8\% \\
% Completion time (ms) & 4420 $\pm$ 138 & 4562 $\pm$ 144 & 4523 $\pm$ 139 & 4602 $\pm$ 150 & 4536 $\pm$ 136 & 4824 $\pm$ 166 & 4747 $\pm$ 144 \\
% \bottomrule
% \end{tabular}
% \label{tab:formal_task2}
% % \vspace{-3mm}
% \end{table*}

\subsection{\yuanjun{Results Analysis}}
% Objective
\noindent\textbf{H1:}
\looseness=-1
We assume that all other sampling strategies perform better than random sampling in preserving relative region density.
% This hypothesis \doc{was} rejected.


\revision{
\textbf{H1} is rejected as random sampling performs the best in preserving relative region density.
}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/formal_task2_new.pdf}
\vspace{-6mm}
\caption{Average accuracy and completion time of \textbf{E2} (Perception of relative class density preservation).
%Error bars indicate 95\% confidence intervals.
}
\vspace{-3mm}
\label{fig:formal_task2}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/DAG_task2_rev.pdf}
\vspace{-8mm}
\caption{Graphical depiction of the pairwise significance relationships of the completion time differences of the sampling strategies in \textbf{E2}.}
\label{fig:DAG_task2}
\vspace{-7mm}
\end{figure}

\begin{figure}[t]
\centering
% \vspace{-5mm}
\includegraphics[width=\linewidth]{fig/formal_task3_new.pdf}
\vspace{-6mm}
\caption{Precision and recall of \textbf{E3} (Perception of outlier maintenance).
% Error bars indicate 95\% confidence intervals.
}
\vspace{-3mm}
\label{fig:formal_task3}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/DAG_task3_rev.pdf}
\vspace{-8mm}
\caption{Graphical depiction of the pairwise significance relationships of the recall differences of the sampling strategies in \textbf{E3}.}
\vspace{-7mm}
\label{fig:DAG_task3}
\end{figure}

% \looseness=-1
Fig.~\ref{fig:formal_task1} shows the results of \textbf{E1}.
\revision{Among all sampling strategies, the accuracy ranges from $94.8\%$ to $98.7\%$, while the average completion time ranges from 2,855ms to 3,283ms.}
Random sampling has the highest accuracy ($98.63\%$) \yuanjun{and the shortest completion time ($2904ms$)} in \textbf{E1}.
%Random sampling also outperforms all other sampling methods in terms of average completion time.
The Friedman tests show that statistical significance \yuanjun{among} different sampling strategies exist in terms of accuracy ($\chi^2(6)=13.56, p = 0.0349$) and average completion time ($\chi^2(6)=20.28, p = 0.0025$).
% in \textbf{E1}
Fig.~\ref{fig:DAG_task1_acc} \yuanjun{depicts} the pairwise significance relationships between each pair of sampling strategies in terms of accuracy.
% demonstrates
Random sampling performs significantly better than multi-class blue noise sampling ($p = 0.0051$) and outlier biased density based sampling ($p = 0.0232$) in terms of accuracy.
Fig.~\ref{fig:DAG_task1_time} \yuanjun{depicts} the pairwise significance relationships in terms of average completion time.
% presents
Random sampling performs significantly better than multi-view Z-order sampling ($p = 0.0328$), multi-class blue noise sampling ($p = 0.0011$), outlier biased density based sampling ($p = 0.0221$), and recursive subdivision based sampling ($p = 0.0048$) in terms of average completion time.
No sampling strategy performs significantly better than random sampling, either in terms of accuracy or average completion time.
% \jiazhi{either}
%The pairwise significance relationships of the sampling strategies are depicted in Fig.~\ref{fig:DAG_task1_acc} and~\ref{fig:DAG_task1_time}.
%Random sampling shows significant difference with multi-class blue noise sampling ($p = 0.0051$) and outlier biased density based sampling ($p = 0.0232$) in accuracy.
%And it shows significant difference with multi-view Z-order sampling ($p = 0.0328$), multi-class blue noise sampling ($p = 0.0011$), outlier biased density based sampling ($p = 0.0221$), and recursive subdivision based sampling ($p = 0.0048$) in completion time.
%Such results explain that random sampling performs better than some other sampling strategies in relative region density preservation, thus rejecting \textbf{H1}.

\noindent\textbf{H2:}
We assume that multi-class adapted sampling strategies, including multi-class blue noise sampling, multi-view Z-order sampling, and recursive subdivision based sampling, perform better than random sampling, blue noise sampling, \yuanjun{density biased sampling} and outlier biased density based sampling in preserving relative class density.

\revision{
\textbf{H2} is partially confirmed as multi-class sampling strategies achieve higher accuracy except for blue noise sampling, while random sampling performs the best in terms of completion time.
}

The results of \textbf{E2} are displayed in Fig.~\ref{fig:formal_task2}.
Blue noise sampling has the highest accuracy at $93.75\%$.
The accuracies of recursive subdivision based sampling ($93.69\%$), multi-class blue noise sampling ($92.06\%$), and multi-view Z-order sampling ($91.75\%$) are higher than the remaining three strategies.
\revision{With an accuracy range of nearly $4\%$ ($89.81\%$--$93.75\%$),}
\doc{however, no significant difference in accuracy is reported using the Friedman test} ($\chi^2(6)=4.019, p = 0.6741$).
%However, difference significance is not found in accuracy according to the Friedman test
%We can see that except for the three multi-class adapted sampling strategies, blue noise sampling also have a rather high accuracy in \textbf{E2}.
%However, difference significance is not found in accuracy according to the Friedman test ($\chi^2(6)=4.019, p = 0.6741$).
% In Experiment 2, there is no significant difference between the sampling methods in terms of the accuracy.

\looseness=-1
In \doc{terms} of average completion time, random sampling performs the best,
\revision{obtaining a result of 4,437ms, while the worst one, outlier biased density based sampling, is more than 400ms slower.}
%the aspect
The three multi-class adapted sampling strategies \doc{offer} no \doc{clear} advantage \doc{compared to} other strategies.
%present, than
The Friedman test shows that \doc{a} significant difference exists in completion time ($\chi^2(6)=12.78, p = 0.0467$).
Fig.~\ref{fig:DAG_task2} shows the pairwise significance relationships in terms of average completion time.
Random sampling performs significantly better than recursive subdivision based sampling ($p = 0.0221$).
% \yuanjun{outlier biased density based sampling ($p = 0.0095$) and}
Besides testing the hypothesis, we also find that outlier biased \yuanjun{density based} sampling performs significantly worse than density biased sampling \yuanjun{($p = 0.0270$)}, random sampling \yuanjun{($p = 0.0095$)}, and blue noise sampling \yuanjun{($p = 0.0270$)}.

%As for average completion time, random sampling performs the best, while outlier biased density based sampling and recursive subdivision based sampling performs the poorest.
%Significant difference exists in completion time ($\chi^2(6)=12.78, p = 0.0467$), and random sampling outperforms both outlier biased density based sampling ($p = 0.0095$) and recursive subdivision based sampling ($p = 0.0221$).
%Furthermore, blue noise sampling and density based sampling shows significant difference with outlier biased density based sampling in terms of completion time ($p = 0.0261$ for both tests).

% Moreover, In Experiment 2, the average completion time data shows that participants can recognize the per-class density fastest in RS (about $4300ms$), with a medium speed in BNS, DBS, MVZS and MCBNS (about $4500ms$), but slowest in OBDBS and RSBS (more than $4700ms$).
% Likewise, for any pair of sampling methods from the different groups divided above,
% they are statistically highly significant ($p < 0.001$) in the difference of average completion time in the task of per-class density recognition.

% With the fact that random sampling can always keep the proportion of points by classes and by regions statistically, we think such preservation of density can be best perceived by human.
% Theoretically, RS can keep the proportion of points of different classes in the same region so that it performs the best.

% \begin{table*}[t]
% \centering
% \caption{Outlier preservation ratio for each sampling method on each dataset in the marked region of our testing data. Sampling rate is the expected preservation ratio for the outliers. The highest ratios for each dataset are highlighted in bold.}
% \begin{tabular}{lllllllll}
% \toprule
% Dataset & RS & BNS & DBS & MVZS & MCBNS & OBDBS & RSBS & Sampling rate \\
% \midrule
% \emph{MNIST} & 2.5\% & 6.5\% & 5.0\% & 4.0\% & 10.6\% & 9.0\% & \textbf{24.8\%} & 3.6\% \\
% \emph{Swiss Roll 2D} & 25\% & 87.5\% & 37.5\% & 50\% & 37.5\% & \textbf{87.5\%} & 50\% & 31.6\% \\
% \emph{Swiss Roll 3D} & 15.9\% & 13.6\% & 15.9\% & 20.5\% & 15.9\% & \textbf{31.8\%} & 29.5\% & 16.9\% \\
% \emph{Abalone} & 25\% & 28.1\% & 40.6\% & 37.5\% & 31.3\% & \textbf{46.9\%} & 40.6\% & 26.9\% \\
% \emph{Clothes} & 19.6\% & 25.9\% & 12.7\% & 14.6\% & 24.7\% & 26.6\% & \textbf{34.8\%} & 14.3\% \\
% \emph{Crowdsourced Mapping} & 22\% & 30\% & 28\% & 32\% & 32\% & 52\% & \textbf{54\%} & 23.3\% \\
% \emph{Epileptic Seizure} & 29.8\% & 29.8\% & 12.8\% & 31.9\% & 36.1\% & \textbf{42.6\%} & 34.0\% & 33.0\% \\
% \emph{Condition Based Maintenance} & 25\% & 25\% & 0\% & 12.5\% & 0\% & \textbf{50\%} & 25\% & 25.3\% \\
% \bottomrule
% \end{tabular}
% \label{tab:outlier_ratio}
% % \vspace{-3mm}
% \end{table*}

\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{fig/formal_task4_new.pdf}
\vspace{-5mm}
\caption{Average ranking scores of \textbf{E4} (Perception of overall shape preservation).
% Error bars indicate 95\% confidence intervals.
}
\vspace{-5mm}
\label{fig:formal_task4}
\end{figure*}

\noindent\textbf{H3:}
We assume that outlier biased density based sampling is the best in preserving outliers.

\revision{
\textbf{H3} is partially confirmed as recursive subdivision based sampling and outlier biased density based sampling achieve higher recall than other strategies, while blue noise sampling has the highest precision.
}

As shown in Fig.~\ref{fig:formal_task3}, outlier biased density based sampling is \doc{ranked fourth} in terms of precision.
%at the
Blue noise sampling, multi-class blue noise sampling, and recursive subdivision based sampling have higher precision than outlier biased density based sampling.
\revision{The precision data span more than $10\%$ ($82.45\%$--$92.98\%$) among all strategies.}
However, the Friedman test \doc{finds} no significant differences in \doc{the precision} of the sampling \yuanjun{strategies} ($\chi^2(6) = 10.53, p = 0.1040$).
In \doc{terms} of recall, outlier biased density based sampling is ranked second, while recursive subdivision based sampling has the highest recall.
% the aspect, at the
% \yuanjun{As listed in Table~\ref{tab:outlier_ratio}, outlier biased density based sampling and recursive subdivision based sampling tend to sample more outliers, which contributes to their high recall.} -> discussion
\revision{The range of recall is about $26\%$, from $23.08\%$ to $49.12\%$, and}
the Friedman test shows that significant differences exist ($\chi^2(6) = 18.78,  p = 0.0045$).
The post-hoc tests show that outlier biased density based sampling performs significantly better than random sampling and density based sampling (Fig.~\ref{fig:DAG_task3}).
Fig.~\ref{fig:DAG_task3} shows the discovered pairwise significance relationships.
\doc{In addition to} the hypothesis test, we also \doc{find} some \doc{other} interesting \doc{results}.
% Besides, have, findings
First, blue noise sampling has the highest precision and the third-highest recall.
Although it has no significance relationship with other strategies in terms of precision and recall, it is worth \doc{recommending it for} outlier preservation \yuanjun{along with outlier biased density based sampling and recursive subdivision based sampling}.
%to be recommended, in the scenario of
In contrast, random sampling and density biased sampling have relatively lower precision and recall than \doc{the} other strategies.
Significance difference\lingyun{s} \doc{are found to} exist between them and outlier biased density based sampling, multi-class blue noise sampling, and recursive subdivision based sampling.

% As shown in Table~\ref{tab:formal_task3}, in Experiment 3, we can find that BNS, MCBNS, and RSBS have much higher precision with the other sampling methods, which is also statistically significant with the Wilcoxon tests.
% We discover that what these three sampling methods have in common is that the points in their sampling results usually separate better and with fewer clutters.
% Such an advantage accounts for their good performance in precision.
%As shown in Fig.~\ref{fig:formal_task3}, generally, all other sampling methods have a comparably higher precision than random sampling and density biased sampling, while recursive subdivision based sampling gets highest recall.
%However, through Friedman tests we find that there is no significant differences in the presicion of the sampling methods ($\chi^2(6) = 10.53, p = 0.1040$).
%In regard to recall, significant differences exist ($\chi^2(6) = 18.78,  p = 0.0045$).
%The results of post-hoc tests show that recursive blue noise sampling, outlier biased density based sampling and blue noise sampling outperform other sampling methods in recall.
%The results of pairwise comparison for recall an be found in Fig.~\ref{fig:DAG_task3}
%Considering the average recall and the significance relationships comprehensively, recursive subdivision based sampling and outlier biased density based sampling are among the best in preserving outliers.
%\textbf{H3} is also partially confirmed by the experiment results.
%As listed in Table~\ref{tab:outlier_ratio}, outlier biased blue noise sampling and recursive subdivision based sampling tend to sample more outliers, which contributes to their high recall.
% while the precision of them was also comparable or even higher than other sampling methods
% Besides, the highest precision of blue noise sampling also makes it obtain a rather high recall compared to other sampling methods except for the two methods above.

\noindent\textbf{H4:}
We assume that blue noise sampling and multi-class blue noise sampling perform better than other strategies in preserving the overall shape.
% This hypothesis is \yuanjun{also partially} confirmed by the subjective experiment \textbf{E4}.

\revision{
\textbf{H4} is also partially confirmed as blue noise sampling gets the highest score, but multi-class blue noise sampling only ranks 4th.
}

Fig.~\ref{fig:formal_task4} shows the average ranking scores of sampling strategies in eight datasets and their average.
Blue noise sampling has the highest ranking score in all eight datasets \yuanjun{with} an average score of $6.37$, \yuanjun{while the performance of multi-class blue noise sampling is \doc{near the middle}}.
% about average}.
%  \jiazhi{in middle level.}
%approximately
\yuanjun{Moreover,} recursive subdivision based sampling, outlier biased density based sampling, and multi-class blue noise sampling has similar \doc{scores} and \doc{rank} 2nd, 3rd, and 4th \yuanjun{with \doc{averages} of $4.82$, $4.74$, and $4.27$}, respectively.
%ranking, at the, scores
The ranking is stable across \doc{all} eight datasets.

% \looseness=-1
\noindent
\revision{
\textbf{Takeaways}.
Since blue noise sampling has competitive results in all experiments, it is suggested to be more generally used in data exploration.
Random sampling performs comparatively well in both E1 and E2, indicating that it is still a competitive choice when users seek to preserve the relative density in the sampled scatterplot given its simplicity.
In addition, as outlier biased density based sampling and recursive subdivision based sampling show their capabilities in outlier maintenance and shape preservation, users may pay more attention to them when encountering such practical needs.
}
%Fig.~\ref{fig:formal_task4} shows the average ranking collected in \textbf{E4}.
%The seven evaluated sampling methods can also be roughly divided into three levels according to their average rankings.
%\textbf{H4} is verified as blue noise sampling outperforms other methods and has an average score of approximately $6.3$.
%Next, outlier biased density based sampling, multi-class blue noise sampling, and recursive subdivision based sampling have an average score of about $4.5$.
%The rest of the sampling methods have an average ranking of about only $2.5$.
% In the contrary, the sampling results of RS, DBS, and MVZS may drop many boundary points so that they have an average ranking of about only $5.5$.
%Moreover, we can see that similar performances are obtained over all the datasets, which further demonstrates the generality of the results.

% \subsection{Subjective Results Analysis}
% \yuanjun{Comment: to be merged with discussion}

% Here we discuss the visual factors that most affect the participants' perception of relative density, outliers, and overall shapes.
% More than half of them mentioned that the distributed area and \yuanjun{the distances between samples} affect their judgments on the region density in \textbf{E1}.
% % With this feedback, we could indicate the reason why blue noise sampling also performed better than many other sampling methods in accuracy in \textbf{E1}.
% % In our data, we found density difference between different regions was not so large that the relative global density can be roughly estimated by the visual factors above.
% % They could best estimated the distributed area and the local density in BNS since it would sample points that were more evenly distributed.
% As for class density recognition, in addition to the previous mentioned factors, participants said that the color and the distribution of the two classes to be compared would also affect their judgments.
% % We found that the sampling strategies where participants spent most time in \textbf{E2}, outlier biased density based sampling and recursive subdivision based sampling, also selected most outliers.
% % This indicated that they would need more time to recognize the points of certain classes in a region containing too many outliers in the sampling results. -> move to discussion
% % This accounts for the longest average completion time of outlier biased density based sampling and recursive subdivision based sampling in \textbf{E2}.
% In \textbf{E3}, some researchers suggested that the continuity of the points of a class would influence their judgments of whether a point was located in the main distribution of its class, thus affecting their judgments of outliers.
% Lastly, people commented that when comparing the preservation of overall shapes, the outline, the hollows, and the size of the shapes are the most important visual factors in their criterion.
% % More uniformly distributed samples can better preserve the outline and the size of the overall shapes, while they can also avoid the occurence of false hollows due to inhomogeneous density.
% % Such feedback is consistent with our observation in \textbf{E3}.

% We also collected the visual factors that participants would be most concerned about sampling in the questionnaire.
% The result is displayed in Fig.~\ref{fig:visual_factor}.
% For the three visual factors evaluated in our experiments, participants favored preserving overall shapes most in the sampling for scatterplots, then relative density, and outliers last.
% They also pointed out that such rating greatly depends on the specific analysis tasks in practical use.
% Besides, when asked for other important visual factors, fifteen of them mentioned that they were interested in the areas where points of different classes mix with each other, while another three participants would focus on the clutter degree in these areas specifically.

% The feedback on the experiments about the influence factors helps us better understand the performance of the participants in the experiments, which is also beneficial to the further experiment design.
% Besides, the rating results on our three selected visual factors confirm that the evaluation targets of our experiments make sense, while the extra important visual factors raised by participants may shed light on new design requirements of sampling.
% Both of them are helpful to develop sampling methods from a perception-driven perspective.


==> Evaluation of Sampling Methods archive/7-discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% 1) Results may differ between automatic evaluation by numerical measures and user study main depends on human perception. (jiazhi)

% 2) Why we only consider sampling on 2D data? (jiazhi)
%     2.1) In recent years, sampling techniques mostly consider 2D data
%     2.2) High dimensional sampling techniques can be also applied to 2D data
%     2.3) On 2D data, tasks can be simplified. We can provide scatterplots before and after sampling and conduct user studies on MTurk
%     2.4) Future work: evaluation of High dimensional sampling techniques

% 3) Color will affect human perception on the global densities in task 1. How to measure or eliminate such effect? What kind of effect will color bring to this experiment?

% 4) The rendering order of points will also affect the perception of the scatterplots. (i.e. if outliers are sheltered, people may consider the sampling is not sufficient)

% \noindent\textbf{Reflection on the experiment design.}
% % As mentioned previously, color will slow down the human perception of relative region density.
% % According to the von Bezold spreading effect~\cite{albers2013interaction}, different color will be wrongly perceived when they are mixed together.
% % This will possibly weaken human perception of certain visual factors in the clutter regions (e.g. density and outliers), thus affecting the performance of the sampling strategies in the correspoding experiments.
% In the subjective questionnaires, participants pointed out many factors that affected their perception of certain visual factors.
% For instance, the overlap of the rendered points may hide some outliers in the sampling results in \textbf{E3}.
% However, it is beyond the acceptable scale of the experiments if including so many factors.
% Although it is a limitation that the experiments do not consider the effect of these factors, we have plentiful trials with different datasets in the experiments so that we can reduce the bias caused by these confounding factors to some extent.

% \yuanjun{Another limitation comes from the composition of our participants.
% The participants we recruited are of better familiarity with scatterplots as well as sampling to guarantee that they fully understand the concepts in the experiments.
% With the trails being relatively simple, participants get experienced with the experiments after some practice trails.
% In this situation, their performances are likely to be at a rather high level than that of visualization practioners with less experience.
% It is also very meaningful to extend our experiments to a wider population of visualization practioners.
% }

% \noindent\textbf{Reflection on the experiment results.}
% When we examined the sampling results of different sampling strategies, we found that outlier biased density based sampling and recursive subdivision based sampling tend to sample more outliers than other sampling strategies.
% In fact, they have the highest outlier retention ratio, and this contributes to their high recall.
% The results in \textbf{E2} show that participants spent most time in relative class density identification with these two sampling strategies.
% It can also be accounted by the observation that the scatterplots of their sampling results look more chaotic with so many outliers.

% In Experiment 4, an interesting finding is that the better-performing sampling method, i.e. blue noise sampling, outlier biased density based sampling, multi-class blue noise sampling, and recursive subdivision based sampling, tend to sample the boundary points of a class or between different classes.
% It may contribute to the presevation of overall shapes since such boundary points help to outline the shape of the distribution of the points of each class.

% However, blue noise sampling still stands out because it can produce more evenly distributed points, which prevents discontinuity of the perception on the overall shapes and also avoids the occurence of false hollows due to inhomogeneous density.

% Additionally, we also find that the average completion time per question in Experiments 2 is approximately 1500ms longer than that in Experiment 1 for any sampling methods, indicating that identifying per-class density is a more challenging task than identifying per-class density for people.

% In Experiment 3 we find that OBDBS and RSBS tend to sample more outliers from the original data so that the scatterplots of their sampling results are relatively more chaotic.
% With the observation that participants cost the longest time in these methods in Experiment 2, it can be inferred that people's ability to perceive the per-class density will decrease under this circumstance.
% \noindent\textbf{Reflection on the experiment results.}

% \noindent\textbf{Reflection on the experiment design.}
% We found that the participants' completion time of Experiment 3 was still too long although we have made a trade-off in the experiment design.
% It will be very meaningful to simplify such task while keeping it effective to evaluate different visualizations.
% Another potential problem was that people will have their own criteria for identifying outliers.
% How will such diversity affect their behaviour and performance will also be an interesting topic.

% \noindent\textbf{Future work.}
% In recent years, the newly developed sampling techniques mostly consider 2D data.
% However, as dimension reduction can be a time-consuming process sensitive to the size of data, it will be more efficient to first sample the data and then reduce their dimensionality when sampling and visualizing high-dimensional data.
% Apart from the sampling methods related to the visual space like multi-view Z order sampling and recursive subdivision based sampling, other sampling methods evaluated can be also applied on high-dimensional data.
% A promising future work is to explore the perception effect when high-dimensional data are first sampled and then projected to the 2D scatterplots.


\subsection{Important Visual Factors in Sampling}
\looseness=-1
The subjective questionnaire on the \doc{important} visual factors provided insights into sampling strategy selection in different scenarios.
The results are presented in Fig.~\ref{fig:visual_factor}.
The average ratings of relative density, outliers, and overall shape, are 4.32, 3.76, and 4.37, respectively.
The high ratings confirm that the evaluated visual factors are \doc{common concerns} in scatterplot sampling.
% the
We also \doc{got} interesting findings when considering the difference between participants from different fields.
% have, \doc{results}
\doc{The} participants in visualization and computer graphics rated 4.00 for outliers and 4.23 for overall shape.
Compared to the averages, they \doc{were} more interested in outlier maintenance than \doc{the} participants in other fields.
% are
In contrast, \doc{the} participants in computer vision and deep learning rated 3.39 for outliers, \doc{but} 4.69 for overall shape.
% and, however
The participants commented that they \doc{were} particularly interested in classification and regression tasks, and the overall shape is helpful \yuanjun{in understanding} the pattern of classification and correlation.
% are
The participants in computer graphics paid more attention to relative density preservation with a rating of 4.63.
\doc{This} is because density is important in geometry modeling tasks of computer graphics.
% It
Therefore, we can recommend sampling strategies according to the specific task.
For instance, although people in computer vision and deep learning are not familiar with blue noise sampling, they \lingyun{are} suggested to try it because blue noise sampling performs the best in overall shape preservation.
% \doc{should}
In addition, extra visual factors \doc{were} proposed in the subjective questionnaire.
% are
\lingyun{For instance, }\jiazhi{the position relationship among classes \yuanjun{(\eg, whether two classes are separated or mixed together)} \doc{was} proposed by 15 participants. }
% \textbf{Comments: what is the meaning of preserving position relationship?}
Three participants commented that the trends \doc{regarding} points should also be preserved.
% of
These ideas might shed light on new design requirements for sampling.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/visual_factor_rev.pdf}
\vspace{-5mm}
\caption{The importance rating of the three evaluated visual factors.}
\vspace{-5mm}
\label{fig:visual_factor}
\end{figure}

%Participants' ratings for the three evaluated visual factors are shown in Fig.~\ref{fig:visual_factor}.
%The average ratings of relative density, outliers, and overall shape, are 4.32, 3.76, and 4.37, respectively,
%With such high ratings, we confirm that the evaluated visual factors are important ones in the scenario of sampling for scatterplots.
%However, they also pointed out that such rating depends on the analysis tasks.
%We then investigate the preferences of the participants from different research fields.
%For instance, the participants majoring in visualization or computer graphics rate 4.00 for outliers, while they rate 4.23 for overall shape.
%Compared to the average rating of all participants, we can find that they are more interested in outlier maintenance since outliers are common subjects in visual analysis tasks.
% According to our experiment results, they can use outlier biased density based sampling and recursive subdivision based sampling when outliers are preferred to be more preserved.
%On the contrary, those majoring in computer vision or deep learning rate 3.39 for outliers but 4.69 for overall shape.
%As the coverage of samples rather than outliers usually exerts stronger effect on the performance of prediction models, they are thus more focused on the overall shape preservation that is related to the coverage of samples in some degree.
% So they can pay more attention to blue noise sampling that can best keep the overall shape.
%The participants majoring in computer graphics paid more attention to relative density preservation with a rating of 4.63.
%Our experiments offer some empirical suggestions on the selection of sampling strategies in different scenarios and in different aspects, so they can pay attention to some specific sampling strategies according to their requirements.

%In addition, participants also proposed some extra visual factors that might be considered in sampling.
%Fifteen of them mentioned that they were interested in the relative position of different classes or clusters, while another three participants would focus on the clutter degree in these areas specifically.
%Besides, three of them mentioned that the trends of the points shown in the scatterplots should also be preserved well.
%These ideas might shed light on new design requirements for sampling.

\subsection{Influencing Factors of Perception and Design Considerations for Sampling}
\looseness=-1
The subjective questionnaire also contained factors that affect perceptions during the experiments.
% the, the
These results provided insights \doc{into} \doc{possible revisits of} our experiment design and shed light on sampling strategy design for different tasks.
%to, revisit
In \textbf{E1}, the covering area (by 60\% of the participants) and the distance among points (by 50\% of the participants) \doc{were} reported to affect region density judgments.
% This report is consistent with the occupancy model~\cite{Allk1991}.
\yuanjun{The occupancy model~\cite{Allk1991} shows that how these factors affect human perception of region density on scatterplots, and there are some previous works~\cite{Vos1988, Bertini2006} \doc{that measured the} perceptual density difference of some factors through user studies.}
%measuring
\yuanjun{Bertini~\etal~\cite{Bertini2006} leverage an ad-hoc perception study result and propose a sampling framework to strengthen the perception of relative density differences.}
\yuanjun{Further exploration \doc{of} integrating perceptual effects with sampling strategy design will be an interesting direction.}
%on
% \jiazhi{\textbf{So what?}}
In \textbf{E2}, the covering area, the distance among points, and the colors of two classes (25\%) \doc{were} reported to be effective visual factors \doc{when making} class density judgments.
%of
\yuanjun{Specifically, }\yuanjun{56\%} of \doc{the respondents} commented that bright color leads to over-estimation of the density.
%them
% \jiazhi{\textbf{the specific number}}
%Seven participants from visualization pointed out that when it is hard to compare the densities of two given classes, they would prefer the one in high contrast color to surroundings.
In our experiment, we randomly set colors from Boynton's color palette~\cite{Boynton1989} \doc{that} are considered to be almost never confused.
%which
The color issue may be further alleviated by optimizing the color assignments to classes after sampling like Wang~\etal~\cite{wang2019optimizing}.
In \textbf{E4}, \yuanjun{66\%} of participants commented that the outline of the shape \doc{was} the most important visual factor when comparing overall shapes.
% over 60\%
% \jiazhi{\textbf{Comments: the specific percentage}}
Inspired by this report, a sampling strategy \doc{aimed} at overall shape preservation should pay more attention to the boundary of clusters.


%In the subjective questionnaires, participants talked about the factors that affected their perception of certain visual factors.
%As the occupancy model~\cite{Allk1991} suggests, 60\% of participants mentioned that the covering area affect their judgments on the region density in \textbf{E1} and 50\% of participants mentioned the distances between samples.
%There are sampling methods seeking to preserve relative densities, but mostly they solve this from a data perspective.
%Such feedback inspires us to refine sampling methods by considering the covering area of samples and their distances to strengthen the perception of relative densities.
%For class density recognition, in addition to the previous mentioned factors, 25\% of participants said that the colors of the two classes to be compared would also affect their judgments.
%Most of them thought bright colors made them overestimate the density, while seven participants from visualization even pointed out that they favored the class with high contrast color with surroundings when it was hard to make a decision.
%Moreover, we also discover that participants spent longest time in \textbf{E2} with outlier biased density based sampling as well as recursive subdivision based sampling, whose sampling results are cluttered in color because of excessive outliers.
%This problem may be addressed by optimizing the color assignments to classes after sampling like~\cite{wang2019optimizing}.
%In \textbf{E3}, six researchers majoring in visualization or computer vision proposed that the continuity of classes would influence their judgments of whether a point was located in an abnormal position, thus affecting their judgments of outliers.
%Recall that participants achieve the best precision in identifying outliers with blue noise sampling and multi-class blue noise sampling; we discover their sampling results also best keep such continuity.
%This observation enlightens us to consider the continuity of classes to enable people to judge outliers more accurately while sampling more outliers when developing outlier-preserving sampling methods.
%Lastly, over 60\% of participants commented that when comparing the preservation of overall shapes, the outlines are the most important visual factors in their criterion, followed by the hollows and the sizes.
%Specifically, six out of thirteen participants majoring in computer vision mentioned that they would consider the relative position of the classes in \textbf{E4}.
%An interesting finding is that in \text{E4}, the better-performing sampling method, i.e. blue noise sampling, outlier biased density based sampling, multi-class blue noise sampling, and recursive subdivision based sampling, tend to sample the boundary points of a class or between different classes, thus better depicting the outlines.
%From the perspective of perception, in order to better preserve the overall shapes, it will make sense to design sampling methods to preserve such boundary points.

\subsection{Limitations and Future Work}
\looseness=-1
As mentioned above, there are many factors affecting the perception of the evaluated visual factors.
On the one hand, these factors, for example, the color in \textbf{E2}, may introduce perceptual bias in our experiments.
Considering that we have a \doc{large} number of trials, \yuanjun{such} bias can be reduced by random settings for the trails.
%this kind of
% considerable
On the other hand, understanding the relationships between them and \doc{the} visual factors \doc{we are concerned with} would be inspiring for \doc{future} sampling strategy design.
However, a controlled experiment containing all \doc{of} these variables would \doc{make it hard to \lingyun{conduct}} a practical evaluation.
% be beyond 
It would be interesting to perform further evaluation of the relationships among them.

%As mentioned above, there are many factors affecting the perception of the evaluated visual factors.
%However, it is beyond the acceptable scale of our experiments if including all of them.
%It is a limitation that the experiments do not consider and analyze the effect of these factors, but we have plentiful trials with different datasets in the experiments so that we can reduce the bias caused by these confounding factors to some extent.
%It will be interesting to explore how to reduce perceptual bias caused by these factors in sampling.

\looseness=-1
In addition, our evaluation only considered sampling on 2D data.
However, scatterplots are usually employed to visualize high-dimensional data \doc{in conjunction with} dimensionality reduction approaches.
% with the companion of
Sampling is performed in the high-dimensional space rather than 2D space for efficiency.
A promising future direction is to explore the perception effects of sampling strategies when they are performed in the high-dimensional space.

%Besides, in recent years, the newly developed sampling techniques mostly consider 2D data.
%However, as dimension reduction can be a time-consuming process sensitive to the size of data, it will be more efficient to first sample the data and then reduce their dimensionality when processing high-dimensional data.
%Apart from the sampling methods related to the visual space like multi-view Z order sampling and recursive subdivision based sampling, other sampling methods evaluated can be also applied on high-dimensional data.
%A promising future work is to explore the perception effect when high-dimensional data are first sampled and then projected to the 2D scatterplots.




==> Evaluation of Sampling Methods archive/abstract.tex <==
\abstract{
% Given a scatterplot with tens of thousands of points or even more, a natural question is which sampling method should be used to create a small but "good" scatterplot for better approximating the original one.  
Given a scatterplot with tens of thousands of points or even more, a natural question is which sampling method should be used to create a small but "good" scatterplot for a better abstraction. 
% approximation
We present the results of a user study that investigates the influence of different sampling strategies on multi-class scatterplots. 
The main goal of this study is to understand the capability of sampling methods in preserving the density, outliers, and overall shape of a scatterplot.
% these
To this end, we comprehensively review the literature and select seven typical sampling strategies as well as eight representative datasets.
We then design four experiments to understand the performance of different strategies in maintaining: 1) \yuanjun{region} density; 2) \yuanjun{class density}; 3) outliers; and 4) overall shape in the sampling results. 
% 1) overall density; 2) relative density among different classes;
The results show that: 1) \yuanjun{random sampling is} preferred for preserving region density; 2) blue noise sampling and random sampling have comparable performance \yuanjun{with the three multi-class sampling strategies} in preserving class density; 3) \yuanjun{outlier biased density based sampling, recursive subdivision based sampling, and blue noise sampling} perform the best in keeping outliers; and 4) \yuanjun{blue noise sampling} outperforms the others in maintaining the overall shape of a scatterplot. 
}
% keeping more outliers

\keywords{Scatterplot, data sampling, empirical evaluation.}



==> Evaluation of Sampling Methods archive/conclusion.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Conclusion}
\label{sec:conclusion}

\looseness=-1
In this paper, we present an empirical evaluation of sampling strategies for scatterplots from the perspective of perception.
We identify seven representative sampling strategies and three critical visual factors for scatterplots following a comprehensive survey \doc{of} the existing literature.
%on
Based on the results, we formulate four hypotheses and design four experiments to evaluate the ability of the selected sampling strategies to preserve the identified visual factors.
We first conduct a pre-study to determine the proper sampling number of each dataset and confirm the negative effect on region density identification caused by color.
The results of the formal study show that (1) random sampling is the best in region density preservation in terms of time and accuracy; (2) blue noise sampling and multi-class sampling strategies \doc{are accurate at} class density preservation, while random sampling \doc{is highly efficient at} this task; (3) recursive subdivision based sampling, outlier biased density based sampling, and blue noise sampling are favored in outlier maintenance; \doc{and} (4) blue noise sampling is the best in overall shape preservation.
% obtain high accuracy/efficiency
These results offer practical guidance for the selection of sampling strategies in different application scenarios.
%\doc{guide}
% \doc{Additionally}, we \doc{survey} the subjective experience of the participants in the formal study and explore the possible directions for the design of sampling strategies from the perspective of perception.
%Besides, collect
% In the future, we plan to investigate the perceptual performances of sampling strategies in the high-dimensional space, and we expect this work will inspire more evaluation studies focusing on sampling, which will make it more effective \doc{at} big data visualization.


==> Evaluation of Sampling Methods archive/method_selection.tex <==

\section{Selection of Sampling Methods}
\label{sec:DataVisSystem}
1) The process of our survey

2) The categorization of our sampling methods (orthogonal categories, jiazhi)
    2.1)single class / multi class
    2.2)uniform probability / non-uniform probability
    
3) Use automatic numerical measures to select sampling methods that perform well


==> method_selection.tex <==

\section{Selection of Sampling Methods}
\label{sec:DataVisSystem}
1) The process of our survey

2) The categorization of our sampling methods (orthogonal categories, jiazhi)
    2.1)single class / multi class
    2.2)uniform probability / non-uniform probability
    
3) Use automatic numerical measures to select sampling methods that perform well

